Fault-Tolerant Labeling and Compact Routing Schemes

The paper presents fault-tolerant (FT) labeling schemes for general graphs, as well as, improved FT routing schemes. For a given $n$-vertex graph $G$ and a bound $f$ on the number of faults, an $f$-FT connectivity labeling scheme is a distributed data structure that assigns each of the graph edges and vertices a short label, such that given the labels of the vertices $s$ and $t$, and at most $f$ failing edges $F$, one can determine if $s$ and $t$ are connected in $G \setminus F$. The primary complexity measure is the length of the individual labels. Since their introduction by [Courcelle, Twigg, STACS '07], compact FT labeling schemes have been devised only for a limited collection of graph families. In this work, we fill in this gap by proposing two (independent) FT connectivity labeling schemes for general graphs, with a nearly optimal label length. This serves the basis for providing also FT approximate distance labeling schemes, and ultimately also routing schemes. Our main results for an $n$-vertex graph and a fault bound $f$ are: -- There is a randomized FT connectivity labeling scheme with a label length of $O(f+\log n)$ bits, hence optimal for $f=O(\log n)$. This scheme is based on the notion of cycle space sampling [Pritchard, Thurimella, TALG '11]. -- There is a randomized FT connectivity labeling scheme with a label length of $O(\log^3 n)$ bits (independent of the number of faults $f$). This scheme is based on the notion of linear sketches of [Ahn et al., SODA '12]. -- For $k\geq 1$, there is a randomized routing scheme that routes a message from $s$ to $t$ in the presence of a set $F$ of faulty edges, with stretch $O(|F|^2 k)$ and routing tables of size $\tilde{O}(f^3 n^{1/k})$. This significantly improves over the state-of-the-art bounds by [Chechik, ICALP '11], providing the first scheme with sub-linear FT labeling and routing schemes for general graphs.

==> intro.tex <==
\section{Introduction}
Distributed graph representation is concerned with augmenting each vertex (and possibly also edges) with useful and low-space information in order to efficiently address various graph queries in a distributed manner. As the
vertices and edges of the network may occasionally fail or malfunction, it is desirable
to make these representations robust against failures. In this paper, we provide new constructions of succinct \emph{labeled-based distributed data structures} that can handle connectivity, distance queries and routing in the presence of edge failures. 

Connectivity labels are short names attached to each vertex in the $n$-vertex input graph $G$, such that given the labels of a pair of vertices $s$ and $t$ (and no any other information), it is possible to deduce if $s$ and $t$ are connected in $G$. The primary complexity measure of the  labeling scheme is the label length (maximum length of a label). In general, labels can be viewed as the \emph{logical} names of the vertices \cite{kannan1992implicat,peleg2005informative}, as they are considerably more informative than the physical names that usually correspond to arbitrary $O(\log n)$-bit identifiers. For example, in routing applications the label of the vertex is treated as its ``address". It is quite immediate to provide connectivity labeling schemes of logarithmic length. Over the years, these labels have served the basis for devising also approximate distance labels, and compact routing schemes, which are arguably the \emph{grand finale} of the distributed representation schemes. 
%Roughly speaking, in the routing setting, the labels of the vertices are used to compute the next hop neighbor on some (possibly approximate) shortest path towards the target.

Our goal in this paper is to provide \emph{fault-tolerant} analogs for the above mentioned schemes, while paying a small overhead in terms of space and other complexity aspects. Fault-tolerant (FT) connectivity labeling scheme, also known in the literature as \emph{forbidden-set} labeling \cite{CourcelleT07}, assigns labels to the vertices and the edges of the graph such that given the labels of a vertex pair $s,t$, and the labels of the faulty edges $F$, one can determine if $s$ and $t$ are connected in $G \setminus F$. Several notions of fault-tolerant labeling and routing schemes have been addressed in the literature; starting with the earlier introduction of FT routing schemes by Dolev \cite{dolev1984new}, to the more recent formulations of forbidden-set labeling and routing schemes by Courcelle et al. \cite{courcelle2007forbidden,CourcelleT07}. Despite much activity revolving these topics, FT labeling and routing schemes with \emph{sub-linear} space are currently known only for a limited collection of graph families. We next elaborate more on the state-of-the-art affairs, and our main objectives. \mtodo{the discussion of related work in the next few pages is quite long. We can consider to have a shorter intro, mainly defining the main problems addressed, and have later a detailed related work section.}

 %including graphs with bounded treewidth, bounded dimension and planar graphs.
%As labeling scheme serves a natural basis for routing schemes, our knowledge the latter is also limited. Specifically, the current FT routing schemes still suffer from suboptimal space vs. stretch tradeoff, using routing tables of possibly super-linear size.

%
%
 %
%To perform also routing in the presence of faults, the FT-connectivity labels should be extended to report also approximate distances, as well as to output the next hop neighbor on the approximate shortest path towards the target. In the standard (fault-free) setting, connectivity labeling scheme with $O(\log n)$ label lengths, are by now a folklore. These labels serve the basis for providing approximate distance labeling, and eventually also compact routing schemes. Since the communication networks are operated in a distributed manner which are subject to local faulty events, it is desirable to devise compact fault-tolerant labeling and routing schemes. Fault-tolerant labeling (and routing) have been studied in the literature under several different terminologies (e.g., forbidden-set labeling, sensitive labeling etc.). Yet to this date, efficient constructions are only known for a limited collection of graph families such as graphs with bounded treewidth, bounded dimension and planar graphs. The problem of devising efficient FT schemes for general graphs (e.g., FT-connectivity labels of \emph{sub-linear} label length) has remains fairly open since the introduction of the FT routing setting by Dolev \cite{dolev1984new}. 

\paragraph{Fault-Tolerant Connectivity Labeling.} FT labels for connectivity were introduced by \cite{courcelle2007forbidden} \mtext{under the term \emph{forbidden-set labeling}. Forbidden set refers to a subset $F$ of at most $f$ edges, such that given the labels of $s,t$ and $F$ one should determine if $s$ and $t$ are connected in $G \setminus F$. The forbidden edge set can be treated in this context as faulty edges\footnote{For routing, the forbidden-set scheme is slightly weaker than FT scheme as explained later.}.} \mtodo{not sure that this is the best place for discussing the forbidden-set name, maybe it can fit better in a related work section.} Since their introduction, efficient FT labeling schemes have been devised only for a restricted collection of graph families. \textbf{MP: For example, Courcelle et al. \cite{CourcelleT07} presented a labeling scheme with logarithmic label length for the families of $n$-vertex graphs with bounded clique-width, tree-width and planar graphs. For $n$-vertex graphs with doubling dimension at most $\alpha$, Abraham et al. \cite{AbrahamCGP16} designed FT labeling schemes with label length $O((1 + 1/\epsilon)^{2\alpha}\log n)$ that output $(1+\epsilon)$ approximation of the shortest path distances under faults.} In the lack of any FT connectivity labeling schemes for general graphs with sub-linear label length (for any $f\geq 2$ faults\footnote{While there is no \emph{explicit} construction of FT labeling for general graphs, for $f=1$, the centralized distance sensitivity oracle of \cite{khanna2010approximate} might be modified to provide approximate distance labels against a single fault.}), we ask:

\begin{question}\label{q:label}
Is it possible to design FT connectivity labeling scheme resilient to at most $f$ edge faults, for general graphs with label length of $\poly(\log n)$ bits, or even $\poly(\log n,f)$ bits? 
\end{question}

\mtodo{The next pargarph is a bit long, we can consider shortning it, and move the more detailed discussion to a related work section. Maybe just focus on the centralized data structures here and not on the certificates?} \mertodo{Yes, I agree, modifying accordingly.} 
%It is noteworthy that the key challenge in our setting is in the \emph{distributed} aspect of the problem, i.e., in \emph{distributively} compressing the graph information to report connectivity queries under any sequence of $f$ faults. For example, in the related sub-graph problem known as \emph{connectivity certificates}, it is known that one can efficiently compute a subgraph $H$ of $O(f n)$ edges that preserves the pairwise connectivity relations under $f$ edge faults \cite{cheriyan1993scan,thurimella1997sub}. This implies that in order to address the collection of all possible $\langle s, t, F \rangle$ connectivity queries (i.e., deciding if $s$ and $t$ are connected in $G \setminus F$), it is sufficient to store only $O(f n\log n)$ bits of information (i.e., storing the edges of the connectivity certificate). 
%These subgraphs can also be computed efficiently in the distributed CONGEST model \cite{Dory18,parter2019small}. 
%but it is unclear how to distribute the information of the $O(f n)$-bit graph information, say roughly ``evenly" among the vertices and the edges, so that FT-connectivity queries can handled efficiently. 
FT connectivity labels are also closely related to \emph{sensitivity connectivity oracles}, which are low-space centralized data-structure that handle efficiently $\langle s, t, F \rangle$ connectivity queries. \textbf{MP: The first construction of these oracles was given by Patrascu and Thorup \cite{patrascu2007planning} providing an $S(n)=\widetilde{O}(fn)$ space oracle that answers $\langle s,t, F \rangle$ connectivity queries in $\widetilde{O}(f)$ time. The state-of-the-art bounds of these oracles are given by Duan and Pettie \cite{DuanConnectivitySODA17}.} 
Our main goal is in providing a \emph{distributed} variant of such constructions, e.g., where each vertex or edge in the graph ``holds" only $S(n)/n$ bits of information, such that an $\langle s,t, F \rangle$ query can be addressed using only the information stored by $s,t$ and $F$. 

\paragraph{Fault-Tolerant Approximate Distance Labeling.} An important step towards designing FT compact routing schemes involves the computation of \emph{FT approximate distance labels}. In this setting, given the labels of $s,t$ and the faulty edges $F$, it is required to report an approximation for the $s$-$t$ shortest path distance in $G \setminus F$. \mtodo{Also the part that starts here may fit better in a related work section (in this case, we will probably need to remove also the question from here - seems that one of the reviwers supported removing the questions in any case).} FT approximate distance labels can be viewed as the distributed analog of $f$-FT \emph{distance sensitivity oracles} \cite{khanna2010approximate,WeimannY10}. 
These are global succinct data-structures that given an $\langle s,t,F \rangle$ query report fast an estimate for the approximate $s$-$t$ distance in $G \setminus F$. \textbf{MP: Chechik et al. \cite{chechik2012f} presented the first randomized construction resilient to $f$ edge faults. 
Specifically, for any $n$-vertex weighted graph, stretch parameter $k$, and a fault bound $f$, they provide a data-structure with $O(f k n^{1+1/k}\log(nW))$ space, query time of $\widetilde{O}(|F|)$, and $O(f k)$ stretch, where $W$ is the weight of the heaviest edge in the graph. Their solution is based on an elegant transformation that converts the FT connectivity oracle of \cite{patrascu2007planning} into an FT approximate distance oracle.} Our goal is to provide FT approximate labeling schemes that match the state-of-the-art space vs. stretch tradeoff provided by the oracles of \cite{chechik2012f}, we ask:

\begin{question}\label{q:dist-label}
Is it possible to design FT approximate distance labels with space vs. stretch tradeoff that match the state-of-the-art bounds of the \emph{centralized} sensitive oracles, e.g., of \cite{chechik2012f}?
\end{question}

\textbf{MP: While the main focus of this paper is in approximate distances, sensitivity oracles that report (possibly near) exact distances under faults have been studied also thoroughly in e.g., \cite{demetrescu2002oracles,bernstein2008improved,duan2009dual,WeimannY10,GrandoniW12,ChechikCFK17,van2019sensitive}. Since reporting exact distances requires linear label length already in the fault-free setting \cite{gavoille2004distance}, we focus on the approximate relaxation, where there is still hope to obtain labels of polylogarithmic length.}
\mtodo{Same comment for this paragraph. Also, there is a recent paper about FT exact distance labels in planar graphs \cite{DBLP:journals/corr/abs-2102-07154} that we should probably mention, they show that any directed weighted planar
graph admits fault-tolerant distance labels of size $O(n^{2/3})$. There are also some references cited in their paper that maybe we should discuss as well, for example see the paragraph ``Forbidden-set distance labeling schemes'' in page 2 here: https://arxiv.org/pdf/2102.07154.pdf} \mertodo{I actually preferred not open up the discussion on special graph families, e.g., planar graphs, graphs with bounded dimension, etc. We do mention it for the direct setting of routing or labeling, but I do not think it should be mentioned for oracles for the following reason. For labels, there was no prior work for general graphs, but for oracles we do have such works so no need to add the extra overhead of special graph families.} 

\paragraph{Fault-Tolerant Routing.} A desirable requirement in most communication networks is to provide efficient routing protocols in the presence of faults. Specifically, an $f$-FT routing protocol is a distributed algorithm that, for any set of at most $f$ faulty edges $F$, allows a vertex $s$ to route a message to a destination vertex $t$ along an approximate $s$-$t$ shortest path in $G \setminus F$ (without knowing $F$ in advance). The routing scheme consists of two algorithms: (i) a preprocessing algorithm which computes (succinct) routing tables and labels for each vertex in the graph; and (ii) a routing algorithm that given the received message and the routing table of vertex $v$ determines the next-hop (specified as a port number) on the $v$-$t$ (approximate) shortest path in $G \setminus F$. The efficiency of the scheme is determined by the tradeoff between: 
\begin{enumerate}[noitemsep]
\item the \emph{stretch} of the route, i.e., the ratio between the length of the route to the $s$-$t$ distance in $G \setminus F$. 
\item the \emph{space} of the routing tables, routing labels and messages. 
\end{enumerate}
While the stretch vs. space tradeoff of routing schemes is fully understood in the non-faulty setting, the corresponding bounds in the FT setting are still far from optimal. \mtodo{Also the part that starts here can fit better in a related work section. Also, a reviwer suggested to discuss also \cite{rajan2012space}. It seems that this work appeard after Chechik et al., and focus on the case of a single edge failure. They show (Theorem 1) a routing scheme with routing tables of size $\widetilde{O}(k \deg(v)+ n^{1/k})$ size per vertex, $O(k^2)$ stretch and $O(k+\log{n})$ size header that handle a failure of one edge.} \textbf{MP: The first formalization of FT routing schemes was given by the influential works of Dolev \cite{dolev1984new} and Peleg \cite{peleg1987fault}. These earlier works presented the first non-trivial solutions for general graphs supporting at most $\lambda$ faulty edges, where $\lambda$ is the edge-connectivity of the graph. Their routing labels had linear size, providing $s$-$t$ routes of possibly linear length (even in cases where the surviving $s$-$t$ path is of $O(1)$ length). In competitive FT routing schemes, it is required to provide $s$-$t$ routes of length that competes with the shortest $s$-$t$ path in $G \setminus F$, even in cases where $G \setminus F$ is not connected. Competitive FT routing schemes \cite{peleg2009good} for general graphs were given by Chechik et al. \cite{ChechikLPR10,chechik2012f} for the special case of $f\leq 2$ faults. 
Specifically, for a given stretch parameter $k$, they gave a routing scheme with a total space bound of $\widetilde{O}(n^{1+1/k})$ bits, polylogarithmic-size labels and messages, and a routing \emph{stretch} of $O(k)$. 
This scheme was extended later on for any $f$ by Chechik \cite{chechik2011fault}, at the cost of increasing the routing stretch to $O(f^2(f+\log^2 n)k)$.}
So far, in all these prior schemes, the space of the individual routing tables could be linear in the worst case, even when allowing a large stretch bound. This is in strike contrast to the standard (non-faulty) compact routing schemes, e.g., by Thorup and Zwick \cite{thorup2001compact}, which provide each vertex a table of $\widetilde{O}(n^{1/k})$ bits, while guaranteeing a route stretch of $2k-1$. The current large gap in the quality of FT routing schemes compared to their non-faulty counterparts leads to the following question.

\begin{question}\label{q:route}
Is it possible to design $f$-fault-tolerant compact routing scheme for general graphs with \emph{sub-linear} table size and with a sub-logarithmic stretch?
\end{question}

\textbf{MP: A more relaxed setting of FT routing scheme which has been studied in the literature is given by the \emph{forbidden set routing schemes}, introduced by Courcelle and Twigg \cite{CourcelleT07}. In that setting, it is assumed that the routing protocol knows in advance the set of faulty edges $F$. In contrast, in the FT routing setting, the failing edges are a-priori unknown to the routing algorithm,  and can only be detected upon arriving one of their endpoints. Forbidden set routing schemes have been devised to the same class of restricted graph families as obtained for the forbidden set labeling setting \cite{CourcelleT07,AbrahamCGP16,abraham2012fully}.}

%In contrast, in the forbidden-set setting the faulty edges are known at the beginning of the routing procedure. Similarly to forbidden-set labeling, forbidden set routing schemes have also been provided for special graph families, including graphs with bounded tree-width and clique-wideth \cite{CourcelleT07}, bounded doubling dimension \cite{AbrahamCGP16}, and planar graphs \cite{abraham2012fully}.


\input{result.tex}




==> labeling-sketches.tex <==
\subsection{Connectivity Labels Based on Graph Sketches}\label{sec:ftconn-sketch}

\mtodo{I'm not sure if we want to have the statement of the theorem with respect to a tree. Maybe only have a variant with a tree where it's needed (for the routing)}

In this section, we show the following:
\begin{theorem}
For every undirected $n$-vertex graph $G=(V,E)$ and a spanning tree $T \subseteq G$, a positive integer $f$, there is a randomized $f$-FS connectivity labels $\FTConnLabel_{G,T}: V \cup E \to \{0,1\}^{Q}$ of length $Q=O(\log^3 n)$ bits. 
\textbf{MP: add later the computation time of the scheme and the decoding time.}
\end{theorem}
In Section \ref{sec:label-alg}, we present the labeling algorithm which assigns labels based on the notion of graph sketches. In Section \ref{sec:dec-alg} we present the decoding algorithm that given the label information determines if $s$ and $t$ are connected in $G \setminus F$. When the graph $G$ and the spanning tree $T$ are clear from the context, we may omit it and simply write $\FTConnLabel$. 



\subsubsection{The Labeling Algorithm}\label{sec:label-alg}
Given a graph $G$, let $T$ be an arbitrary rooted tree in $G$ that is used throughout this section.
For any node $u \in V(T)$, let $V_u$ be the subset of nodes in the subtree of $T$ rooted at $u$. The algorithm starts by computing ancestry labels $\LCALabel(u)$ for all nodes $u$ given the tree $T$ using Lemma \ref{anc_labels}. Additionally, we assign to all vertices unique ids $\ID(v)$ between $\{1,...,n \}.$

\paragraph{Extended Edge Identifiers.} Each edge $e$ in $G$ is assigned to a unique identifier $ID_T(e)$ that is made of two parts: a \emph{distinguishing} part $ID_{1,T}(e)$ (that does not depend on $T$) and a \emph{logical part} $ID_{2,T}(e)$ that depends on $T$; each of $O(\log n)$ bits. The distinguishing part $ID_{1,T}(e)$ is defined in a way that guarantees that the XOR of several identifiers does not correspond to a legal identifier of any edge $e \in G$ w.h.p. The logical part $ID_{2,T}(e)$ contains auxiliary information that aids the decoding algorithm. 
The computation of the distinguishing parts $ID_{1,T}(e)$ is based on the notion of $\epsilon$-\emph{bias} sets \cite{naor1993small}. The construction is randomized and guarantees that, w.h.p., the XOR of the $ID_{1,T}$ part of each given subset of edges $S \subseteq E$, for $|S|\geq 2$, is not a legal $ID_{1,T}$ identifier of any edge.
%The algorithm will be able to detect whether a given $O(\log n)$ bits corresponding to an $\XOR(S)$ is a legal ID (in which case, $S$ contains a single edge) or not, w.h.p.
Let $\XOR(S)$ be the bitwise XOR of the extended identifiers of edges in $S$, i.e., $\XOR(S)=\oplus_{e \in S} \ID_T(e)$. In addition, let $\XOR_1(S)=\oplus_{e \in S} \ID_{1,T}(e)$.

\begin{lemma}[Modification of Lemma 2.4 in \cite{GhaffariP16}]
\label{cl:epsbias}
There is an algorithm that creates a collection $\mathcal{I}=\{\ID_1(e_1), \ldots, \ID_1(e_{M})\}$ of $M=\binom{n}{2}$ random identifiers for all possible edges $(u,v)$, each of $O(\log n)$-bits using a seed $\mathcal{S}_{ID}$ of $O(\log^2 n)$ bits. These identifiers are such that for each subset $E' \subseteq E$, where $|E'|\neq 1$, we have $\Pr[\XOR_1(E') \in \mathcal{I}] \leq 1/n^{10}$. In addition, given the identifiers $\ID(u), \ID(v)$ of the edge $e=(u,v)$ endpoints, and the seed $\mathcal{S}_{ID}$, one can determine $\ID_1(e)$ in $\widetilde{O}(1)$ time.
\end{lemma}
\begin{proof}
The lemma is proved in \cite{GhaffariP16}, the only part that is not discussed there is the time to determine $\ID_1(e)$ that follows from \cite{naor1993small}. 
By Theorem 3.1 of \cite{naor1993small}, given the seed $\mathcal{S}_{ID}$ and the edge identifier $e_j=(\ID(u), \ID(v))$, determining the $i^{th}$ bit of $\ID_1(e_{j})$ can be done in $O(\log n)$ time. Thus, determining all $O(\log n)$ bits, takes $O(\log^2 n)$ time. 
\end{proof}
The second part of the identifier $\ID_{2,T}(e)$ is given by $\ID_{2,T}(e)=[\ID(u), \ID(v), \LCALabel_T(u), \LCALabel_T(v)]$. 
The identifiers of $\ID_T(u), \ID_T(v)$ are used in order to verify the validity of the first part of the label $\ID_1(e)$. When the tree $T$ is clear from the context, we might omit it and simply write $\ID(e)$. 

\paragraph{Graph Sketches.}
Graph sketches are a powerful tool to identify outgoing edges \cite{kapron2013dynamic,ahn2012analyzing}. \mtodo{I can add some references later, maybe in the related work section} We start by illustrating the intuition behind them. For a vertex $v$, let $\bSketch(v)$ be the bitwise xor of all IDs of edges adjacent to $v$. If we take a subset of vertices $S$, and define  $\bSketch(S) = \oplus_{v \in S} \bSketch(v)$, we can see that all edges that have both endpoints in $S$ are cancelled, and we are left with the xor of outgoing edges from $S$. If there is only one such edge, we get its id. In the case there are more outgoing edges, we can use sampling to identify one outgoing edge. We next formalize this idea and show how to use it in our labels. 

\paragraph{Forbidden-Set Labels via Graph Sketches.} 
The graph sketches are based on random sub-sampling of the graph edges with logarithmic number of scales, i.e., with probability of $2^{-i}$ for every $i \in \{1,\ldots, m\}$. For our purposes and similarly to \cite{DuanConnectivityArxiv16,DuanConnectivitySODA17}, we use pairwise independent hash functions to decide whether to include edges in sampled sets. Choose $L=c\log n$ 
pairwise independent hash functions $h_1, \ldots, h_{L}:\{0,1\}^{2\log n} \to \{0, \ldots, 2^{\log m}-1\}$, and for each $i \in \{1, \ldots, L\}$ and $j \in [0,\log m]$, define the edge set 
$$E_{i,j} =\{ e \in E ~\mid~ h_i(e) \in [0,2^{\log m-j})\}~.$$ 
Each of these hash functions can be defined using a random seed of logarithmic length \cite{TCS-010}. Thus, a 
random seed $\mathcal{S}_h$ of length $O(L \log n)$ can be used to determine the collection of all these $L$ functions. As observed in \cite{DuanConnectivityArxiv16,GibbKKT15}, pairwise independence is sufficient to guarantee that for any set $E' \subset E$ and any $i$, there exists a $j$ such that with constant probability $\XOR(E' \cap E_{i,j})$ is the name (extended identifier) of one edge in $E'$, for a proof see Lemma 5.2 in  \cite{GibbKKT15}.
\begin{lemma}\label{lem:hitting-pairwise}
For any edge set $E'$ and any $i$, with constant probability there exists a $j$ satisfying that $|E' \cap E_{i,j}|=1$.
\end{lemma}


We also need to be able to tell that a bit string of $\XOR(E' \cap E_{i,j})$ is a legal edge ID or not.
\textbf{MP: all these lemmas and claims can (should) be moved to the subsequent analysis section.}

\begin{lemma}
Given the seed $\mathcal{S}_{ID}$, one can determine in $\widetilde{O}(1)$ time if $\XOR(E' \cap E_{i,j})$ corresponds to a single edge ID in $G$ or not, w.h.p.
\end{lemma}
\begin{proof}
Let $X=\XOR(E' \cap E_{i,j})$. Letting $E''=E' \cap E_{i,j}$, then $X$ can be written as the concatenation of $\XOR_1(E'')$ and $\XOR_2(E'')$. 
Using the seed and $\XOR_2(E'')$, one can test the validity of $\XOR_1(E'')$.
The algorithm detects the case that $|E''| \geq 2$ as follows. First, in the case that $E''$ is a single edge, $\XOR_2(E'')$ should contain legal ids $\ID(u),\ID(v)$. If this is not the case, it follows that $|E''| \neq 1$. If $\XOR_2(E'')$ contains legal ids $\ID(u),\ID(v)$, we use them and the seed $\mathcal{S}_{ID}$ to determine $\ID_1(e)$ for $e = (u,v)$, and we check if $\XOR_1(E'')=\ID_1(e)$. We have two options, either $E'' = \{e\}$ is the single edge $e$, in which case $\XOR_1(E'')=\ID_1(e) \in \mathcal{I}$, and the verification succeeds. Otherwise $|E''| \geq 2$, in which case, from Lemma \ref{cl:epsbias}, $\Pr[\XOR_1(E'') \in \mathcal{I}] \leq 1/n^{10}$, hence w.h.p $\XOR_1(E'') \neq \ID_1(e) \in \mathcal{I}$ and we identify that $|E''| \geq 2$.
%To show that the algorithm detects the case that $|E''|\geq 2$, we should show that w.h.p. 
%$$h(u_1,v_1) \oplus h(u_2,v_2) \neq h(u_1 \oplus u_2, v_1 \oplus v_2)$$ \mtodo{is it enough to show it for 2? I think that if we know what are the %original ids (say the set $\{1,...,n\}$), we can get a simpler proof using Lemma 2.9, I'm not sure if we want this assumption.}
%where $h(u,v)$ is $\ID_1(e)$ for $e=(u,v)$. TBD.
\end{proof}
For each vertex $v$ and indices $i,j$, let $E_{i,j}(v)$ be the edges incident to $v$ in $E_{i,j}$. 
The $i^{th}$ \emph{basic sketch unit} of each node $v$ is then given by:
\begin{equation}
\label{eq:vsketch}
\Sketch_i(v)=[\XOR(E_{i,0}(v)),\ldots,\XOR(E_{i,\log m}(v))].
\end{equation}
The sketch of each node $v$ is defined by a concatenation of $L=\Theta(\log n)$ basic sketch units: 
$$\Sketch(v)=[\Sketch_{1}(v),\Sketch_{2}(v), \ldots\Sketch_{L}(v)]~.$$ 
For every subset of vertices $S$, let 
$\Sketch(S)=\oplus_{v \in S}\Sketch(v).$ 

We are now ready to define the forbidden set \mtodo{fault-tolerant?} connectivity labels of vertices and edges. 
The label of each vertex $u$ is given by:
$$\FTConnLabel_{G,T}(u)=\langle \Sketch(V(T(u))), \Sketch(V), \LCALabel_T(u), \mathcal{S}_{ID}, \mathcal{S}_h\rangle,$$ 
where $\LCALabel_T(u)$ is the ancestry label of $u$ with respect to the tree $T$.
The label $\FTConnLabel_{G,T}(e)$ of each \emph{edge} $e=(u,v)$ is as given by:
%\textbf{MP: Suggestion: we may want to have distinct labels for tree edges and non-tree edges, as below. This facilitate the notation for the routing scheme}
\begin{equation*}
    \FTConnLabel(e)=
    \begin{cases}
      \langle \FTConnLabel_{G,T}(u), \FTConnLabel_{G,T}(v)\rangle ,& \mbox{~for~} e \in T \\
     \langle ID_T(e) \rangle,& \mbox{~Otherwise}.
    \end{cases}
\end{equation*}


\begin{claim}
The label length is $O(\log^3 n)$ bits.
\end{claim}
\begin{proof}
The label size is dominated by the sketching information $\Sketch(V_u)$, which is made of a concatenation of the bitwise XOR of $O(\log n)$ basic sketch units $\Sketch_i(u)$. By Eq. (\ref{eq:vsketch}), each unit has $O(\log^2 n)$ bits, and thus overall, the label has $O(\log^3 n)$ bits.
\end{proof}

\mtodo{I think maybe now we want something slightly different, that given a basic sketch unit, we can find with constant probability an outgoing edge? Also, should add a proof.}

\begin{lemma}\label{lem:sketch-property}
For any subset $S$, given $\Sketch(S)$ one can compute, w.h.p., an outgoing edge $E(S, V \setminus S)$ if such exists. 
\end{lemma}


\subsubsection{The Decoding Algorithm} \label{sec:dec-alg}
We next describe the decoding algorithm where given every triplet $s,t, F \in V \times V \times E^f$ along with their labels, it determines whether $s$ and $t$ are connected in $G\setminus F$, w.h.p. For our decoding algorithm it would actually be sufficient to get as input:
\begin{enumerate}[noitemsep]
\item the connectivity labels of $s,t$, the labels of the faulty tree-edge $F \cap E(T)$, and in addition,
\item the extended identifiers of the faulty non-tree edges $F \setminus T$ (which are part of the labels)\footnote{This property will be important later on for obtaining the compact routing schemes.}. 
\end{enumerate}
The decoding algorithm has four key steps: The first step identifies the at most $f+1$ components $\mathcal{C}_0=\{C_1,\ldots, C_\ell\}$ of $T \setminus F$, as well as the components of $s$ and $t$ in $\mathcal{C}_0$. The second step uses the label information to compute the sketch value $\Sketch(C_i)$ of each component $C_i \in \mathcal{C}_0$. The third step modifies this sketch information into $\Sketch_{G \setminus F}(C_i)$, by subtracting the information related to the faulty edges. The forth and final step uses the sketch information in order to simulate $L=O(\log n)$ steps of the Boruvka algorithm. At the end of these steps, the decoding algorithm identifies the connected components of both $s$ and $t$ in $G \setminus F$. In the case where $s$ and $t$ are indeed connected in $G \setminus F$, the algorithm also outputs a succinct representation of an $s$-$t$ path in $G \setminus F$. This extra information would be used later on by our compact routing scheme. We next describe these steps in details. 

\paragraph{Step 1: Identification of the connected components $\mathcal{C}_0$ in $T \setminus F$.} 
Let $F_T=F \cap T$ be the faulty tree edges and let $F_{NT}=F \setminus F_T$ be the faulty non-tree edges. Let $U=\{s,t\} \cup V(F_T)$.  Each component $C_i$ of $T \setminus F$ will be identified by the maximum vertex ID in $C_i \cap U$. Note that the non-tree faulty edges $F_{NT}$ have no impact on the components of $T \setminus F$ (thus their labels are indeed not needed for that step).
We next show that although we do not have full information about the tree $T$ and the vertices of each connected component, the ancestry labels of $V(F_T)$ give us enough information to identify the connected components of $T \setminus F$. Additionally, given an ancestry label of a vertex $u$, we can identify the connected component of $u$. To obtain this, it is helpful to look at the \emph{component tree} that is obtained by contracting each connected component of $T \setminus F$ to one vertex, as follows. Let $\ell = |F_T|+1.$ The component tree $T_C = (\mathcal{C}_0, E_C)$ is a tree of $\ell$ vertices representing the connected components in $T \setminus F$, and $|F_T|=\ell-1$ edges corresponding to the edges of $F_T$. There is an edge $\{C_i,C_j\} \in E_C$ iff there is an edge $\{u,v\} \in F_T$ where $u \in C_i, v \in C_j$. See Figure \ref{componentTreePic} for an illustration.  We can construct the tree $T_C$ using the ancestry labels of the edges $F_T$. For this we just need to identify for any edge in $F_T$ the set of edges from $F_T$ above it in $T$. Moreover, for a given vertex $v$, its connected component is exactly determined by the set of edges in $F_T$ above it in $T$, which can again be identified using the ancestry labels of $v \cup V(F_T)$. In particular, we can identify the connected components of $s$ and $t$. \mtodo{add the time complexity, we can probably get a faster algorithm if needed.}

\setlength{\intextsep}{0pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.55]{componentTree.pdf}
 \caption{Illustration of the component tree where $F=\{e_1,e_2,e_3,e_4\}$. Each connected component of $T \setminus F$ is contracted to one vertex on the right.}
\label{componentTreePic}
\end{figure}
 

\paragraph{Step 2: Computing the sketch values of each component $\mathcal{C}_0$ in $G$.} 
For each component $C_j \in \mathcal{C}_0$ the algorithm computes $\Sketch_G(C_j)$ using the label information of the nodes in $U$.  The basic observation here is the following. Given $S' \subset S$ and $\Sketch(S), \Sketch(S')$, it holds that $\Sketch(S \setminus S')=\Sketch(S) ~\XOR~ \Sketch(S')$. To compute the sketch values, first, we define for each component a temporary value $\Sketch'_G(C_j)$ as follows. Let $v_j$ be the highest vertex in the component $C_j$. For the component of the root $r$, this is $r$. For any other component $C_j$, let $\{C_j,p(C_j)\}$ be the edge connecting $C_j$ to its parent in the component tree. This edge corresponds to an edge $\{v,p(v)\} \in F_T$, where $v$ is the highest vertex in $C_j$. We define $\Sketch'_G(C_j) = \Sketch_G(V_{v_j})$. Note that this value is part of the label of the vertex $v_j$. For any $v_j \neq r$, we have $v_j \in V(F_T)$, and we also learn the identity of $v_j$ when constructing the component tree in Step 1, hence we know $\Sketch'_G(C_j)$. We also know the temporary sketch value of the component of $r$, as $\Sketch_G(V_{r})=\Sketch_G(V)$ is part of the labels of all vertices. We next use the temporary sketch values to compute the sketch values of components using the following claim.

\begin{claim}
Let $C_j$ be a component in $T \setminus F$. If $C_j$ is a leaf in the component tree, we have $\Sketch_G(C_j) = \Sketch'_G(C_j).$ Otherwise, let $D=\{D_1,...,D_t\}$ be the children of $C_j$ in the component tree and let $\Sketch'(D)=\oplus_{1 \leq i \leq t} \Sketch'_G(D_i)$, then $\Sketch_G(C_j) = \Sketch'_G(C_j) \oplus \Sketch'(D).$ 
\end{claim}

\begin{proof}
It holds that $\Sketch_G(C_j) = \oplus_{v \in C_j} \Sketch_G(v)$. By definition, $\Sketch'_G(C_j)=\Sketch_G(V_{v_j}) = \oplus_{v \in V_{v_j}} \Sketch_G(v)$ is the xor of sketches of all vertices in the subtree of $v_j$. As $v_j$ is the highest vertex in $C_j$, if $C_j$ is a leaf component in the component tree, then the vertices in $C_j$ are exactly the vertices in $V_{v_j}$, and the claim follows. Otherwise, the vertices in $C_j$ are all vertices in $V_{v_j}$ that are not contained in any component below $C_j$. Hence, to compute the value $\Sketch_G(C_j)$, we should subtract from $\Sketch_G(V_{v_j})$ the sketch values of vertices in components below $C_j$. Let $D_1,...,D_t$ be the children of $C_j$ in the component tree, and let $u_1,...,u_t$ be the highest vertices in the components $D_1,...,D_t$. Any vertex that is in some component below $C_j$ is in exactly one of the subtrees $V_{u_1},...,V_{u_t}$. Hence the sketch value of vertices in components below $C_j$ equals $\oplus_{1 \leq i \leq t} \Sketch_G(V_{u_i})= \oplus_{1 \leq i \leq t} \Sketch'_G(D_i)=\Sketch'(D)$. To conclude, we get $\Sketch_G(C_j)=\Sketch_G(V_{v_j}) \oplus \Sketch'(D)=\Sketch'_G(C_j) \oplus \Sketch'(D)$, as needed.
\end{proof}

To conclude, from the values $\Sketch'_G(C_j)$, we can easily compute the values $\Sketch_G(C_j)$. The complexity is $\tilde{O}(f)$, as for each component, the sketch $\Sketch'(C_j)$ participates in two computations, and we have at most $O(f)$ components and the sketches have poly-logarithmic size.


\paragraph{Step 3: Computing the sketch values of each component $\mathcal{C}_0$ in $G \setminus F$.} 
For each faulty edge $e \in F$ (both tree and non-tree edges), our goal is to subtract the sketch information of $e$ from the corresponding components of the endpoint of $e$. The step does not require the label information of the edges, and it would be sufficient to know only the seed $\mathcal{S}_h$ that determines the sampling of edges into the sketches, and the extended identifier of the failing edges. 

Using the extended identifier of the faulty edge $e=(u,v)$, one can determine the components in $\mathcal{C}_0$ to which its endpoints belong from the ancestry labels of $u$ and $v$, as explained in Step 1. Using the identifier $\ID(e)$ and the seed $\mathcal{S}_h$, one can determine all the indices of the sketch to which the edge $e$ was sampled. \mtodo{what is the complexity of this? MP: It should be $\widetilde{O}(1)$ using Fact \ref{fc:pairwise}.}
Letting $C_u, C_v$ be the components of $u$ and $v$ in $T \setminus F$, respectively. The values $\Sketch_G(C_u),\Sketch_G(C_v)$ are updated by XORing them with the matrix that contains the identifier $\ID(e)$ in the relevant positions. \mtext{The complexity is poly-logarithmic, as the matrix has poly-logarithmic size.}
From that point on, all sketches of the components $\mathcal{C}_0$ can be treated as sketches that have been computed in $G \setminus F$.  


\paragraph{Step 4: Simulating the Boruvka algorithm.} Finally, our goal is to determine the identifiers of the maximal connected components of $s$ and $t$ of $G \setminus F$. The input to this step is the identifiers of the components $\mathcal{C}_0=\{C_{1}, \ldots, C_k\}$ in $T \setminus F$, along with their sketch information in $G \setminus F$. While the algorithm does not have information on the nodes of each component, it knows the component identifier of each node in $U$. 

The algorithm consists of $L=O(\log n)$ phases of the Boruvka algorithm. Each phase $i \in \{1,\ldots, L\}$ will be given as input a partitioning $\mathcal{C}_i=\{C_{i,1}, \ldots, C_{i,k_i}\}$ of (not necessarily maximal) connected components in $G \setminus F$.
These components are identified by an $O(\log n)$ bit identifier, where for each vertex in $U$, the algorithm receives its unique component identifier in  $\mathcal{C}_i$. In addition, the algorithm receives the sketch information of the components $\mathcal{C}_i$ in $G \setminus F$. The output of the phase is a partitioning $\mathcal{C}_{i+1}$, along with their sketch information in $G \setminus F$ and the identifiers of the components for each node in $U$. A component $C_{i,j} \in \mathcal{C}_i$ is \emph{growable} if it has at least one non-faulty outgoing edge to a node in $V \setminus C_{i,j}$. That is, the component is growable if it is strictly contained in some maximal connected component in $G \setminus F$. Letting $N_i$ denote the number of growable components in $\mathcal{C}_i$, the output partitioning $\mathcal{C}_{i+1}$ of the $i^{th}$ step guarantees that $N_{i+1}\leq N_i /2$ w.h.p. To obtain outgoings edges from the growable components in $\mathcal{C}_i$, the algorithm uses the $i^{th}$ basic-unit sketch $\Sketch_i(C_{i,j})$ of each $C_{i,j} \in \mathcal{C}_i$. By Lemma \ref{lem:sketch-property}, from every growable component in $\mathcal{C}_i$, we get one outgoing edge $e'=(x,y)$ with constant probability. Using the extended edge identifier of $e'$ the algorithm can also detect the component $C_{i,j'}$ to which the second endpoint, say $y$, of $e'$ belongs. Specifically, this is done using the ancestry label of the detected edge $e'$. That label allows us to compute the component of $y$ in the initial partitioning $T \setminus F$, i.e., the component $C_{0,q}$ of $y$ in $\mathcal{C}_0$. Thus $y$ belongs to the unique component $C_{i,j'} \in \mathcal{C}_i$ that contains 
$C_{0,q}$. 


%The algorithm uses the sketch information to compute at least one outgoing edge from each growable component $C_{i,j}$. This is done using the $i^{th}$ block of $K'=O(\log n)$ sketches $\{\Sketch_{(i-1)K+\ell}(C_{i,j}), \ell \in \{1,\ldots, K'\}\}$ to compute an outgoing edge. \mtodo{check indexes, $K$ or $K'$?}

As noted in prior works \cite{ahn2012analyzing,kapron2013dynamic,DuanConnectivityArxiv16}, it is important to use fresh randomness (i.e., independent sketch information) in each of the Boruvka phases. The reason is that the cut query, namely, asking for a cut edge between $S$ and $V \setminus S$, should not be correlated with the randomness of the sketches. Note that indeed the components of $\mathcal{C}_i$ are correlated with the randomness of the first $(i-1)$ basic sketch units of the vertices. Thus, in phase $i$ the algorithm uses the $i^{th}$ basic sketch units of the vertices (which are independent of the other sketch units) to determine the outgoing edges of the components in $\mathcal{C}_i$.

%\begin{claim}\label{cl:balg}
%Given a sketch $\Sketch_i(C_{i,j})$ of a growable compo
%W.h.p given the set of sketches $\{\Sketch_{(i-1)K+\ell}(C_{i,j}), \ell \in \{1,\ldots, K'\}\}$, one can determine an outgoing edge $e=(u,v) \in C_{i,j} \times (V\setminus C_{i,j})$ in time $\widetilde{O}(1)$ if such an edge exists. In addition, one can also compute the component $C_{i,j'}$ such that $v \in C_{i,j'}$ in $\widetilde{O}(1)$ time. 
%\end{claim}
%\begin{proof}
%
%\end{proof}
%By Cl. \ref{cl:balg}, w.h.p. the algorithm computes an outgoing edge from each of the components which leads to a merging of the components. 

The algorithm then computes the updated sketches of the merged components. This is done by xoring over the sketches of the components in $\mathcal{C}_i$ that got merged into a single component in 
$\mathcal{C}_{i+1}$. In expectation, the number of growable components is reduced by factor $2$ in each phase. Thus after $O(\log n)$ phases, the expected number of growable components is at most $1/n^5$, and using Markov inequality, we conclude w.h.p there are no growable components. The final partitioning $\mathcal{C}_L$ corresponds w.h.p to the maximal connected components in $G \setminus F$. The pair $s$ and $t$ are connected in $G \setminus F$ only if the components $C_s,C_t$ of $s,t$ respectively in $T \setminus F$ are connected in the final component decomposition.
\mtodo{add complexity.}

%For simplicity assume first that there is only one failing edge $e=(u,v)$ in $T$. W.l.o.g assume that $v$ is the parent of $u$ in the tree (this can be checked using the LCA labels). The forest $T \setminus \{e\}$ has two components given by $V_u$ and $\bar{V}_u=V \setminus V_u$. The sketch value $\Sketch(V_u)$ and $\Sketch(\bar{V}_u)$ are explicitly stored in the label of $u$ (which is part of $\FTConnLabel(e)$). To update these sketches into sketches in $G \setminus F$ we do as follows. First we cancel the effect of the edge $e$ by using the information stored in $\FTConnLabel(e)$. That is, we add $ID(e)$ to every entry in the sketch $\Sketch(V_u)$ and $\Sketch(\bar{V}_u)$ in which it appears. The cancellation of inter-cluster edges $e' \in F$ is performed in the same manner. 
%
%\begin{description}
%\item add information of LCA to the labels, so that we can detect the LCA label of the edge.
%\item bound the time in which we can tell that the XOR is not a legal edge.
%\end{description}
Finally, we show that the decoding algorithm can be slightly modified to output a compressed encoding of an $s$-$t$ path in $G \setminus F$, using $O(f\log n)$ bits. This encoding is represented by an $s$-$t$ path $\widehat{P}$ that has two type of edges, appearing in an alternate manner on  $\widehat{P}$: $G$-edges and edges $e'=(u,v)$ such that the $u$-$v$ tree path is intact in $T \setminus F$. See Figure \ref{fig:succ-paths}. 
\begin{lemma}\label{lem:useful-recovery-edges}
Consider a triplet $s,t,F$ such that $s$ and $t$ are connected in $G \setminus F$. 
The decoding algorithm can also output a set of at most $f$ recovery edges $Q$ such $(T \setminus F) \cup Q$ is a spanning tree. In addition, it outputs a labeled $s$-$t$ path $\widehat{P}$ of length $O(f)$ that provides a succinct description of the $s$-$t$ path. The edges of $\widehat{P}$ are labeled by $0$ and $1$, where $0$-labeled edges correspond to $G$-edges and $1$-labeled edges $e=(x,y)$ correspond to $x$-$y$ paths in $T \setminus F$. 
\end{lemma}
\begin{proof}
Let $C_s, C_t$ be the components of $s$ and $t$ in the initial partitioning $\mathcal{C}_0$. In Step $4$ of the decoding algorithm, the Boruvka algorithm is simulated up to the point that $C_s$ and $C_t$ are connected. Therefore, the algorithm has computed a path $P$ that connects the components $C_s$ and $C_t$. Each node on that path corresponds to a component in $\mathcal{C}_0$, and each edge corresponds to an outgoing edge (discovered using the sketch information). Since $\mathcal{C}_0$ has at most $f+1$ components, $|P|\leq f+1$. 
Each such edge $e' \in P$ corresponds to an edge in $G$. Let $e_1=(x_1,y_1),\ldots, e_k=(x_k,y_k)$ be the $G$-edges corresponding to the edges of $P$ ordered from $C_s$ to $C_t$. Letting $y_0=s$ and $x_{k+1}=t$, we get that 
$y_i$ and $x_{i+1}$ belong to the same component in $\mathcal{C}_0$, for every $i \in \{0,\ldots, k\}$. 
The labeled path is given by $\widehat{P}=[s, x_1,y_1, x_2, y_2, \ldots y_k,t]$ where the edges $(y_i,x_{i+1})$ are labeled $1$ and the edges $(x_{i}, y_i)$ are labeled $0$. Each $0$-labeled edge is a real edge in $G$, and each $1$-labeled edge $(x_{i}, y_i)$ corresponds to a tree path $\pi(x_i, y_i)$ in $T \setminus F$. 
\end{proof}


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.40]{suc-path.pdf}
\caption{\sf Shown is a tree $T$ with faulty edges $e_1,\ldots, e_4$. The $s$-$t$ path in $G \setminus F$ is represented by the path $\widehat{P}=[s,v_1]\circ (v_1,v_2) \circ [v_2,v_3] \circ (v_3,r) \circ [r,v_4] \circ (v_4, v_5) \circ [v_5,t]$. The recovery edges $(v_1,v_2), (v_3,r)$ and $(v_4, v_5)$ are shown in dashed lines.  \label{fig:succ-paths}
}
\end{center}
\end{figure}

==> routing-scheme.tex <==
\section{Compact Routing Schemes}
In this section, we explain how to use our FT-distance labels to provide compact and low stretch routing schemes. This is the first scheme to provide an almost tight tradeoff between the space and the multiplicative stretch, for a constant number of faults $f=O(1)$.  Throughout this section, tree routing operations are performed by using the tree routing scheme of Thorup and Zwick \cite{thorup2001compact}.
\begin{fact}\label{fc:route-trees}[Routing on Trees]\cite{thorup2001compact}
For every $n$-vertex tree $T$, there exists a routing scheme that assigns each vertex $v \in V(T)$ a label $L_T(v)$ of $(1+o(1))\log n$ bits. Given the label of a source vertex
and the label of a destination, it is possible to compute, in constant time, the port number of the edge from the source that heads in the direction of the destination.
\end{fact}

\textbf{MP: check if needed.} \mtodo{I've added a discussion of the port information later.}
In our routing scheme, each vertex $u$ is required to compute the port number of the next-hop towards the target destination. Towards that goal, we modify the FT-distance labels of Sec. \ref{sec:ft-distance}, by adding the port information to the extended identifier of the edges. That is, the extended identifier of each edge $e=(u,v)$ is augmented with a third field containing the port number of $v$ w.r.t $u$ and vice-versa. To avoid cumbersome notation, we still refer to this port-augmented FT-distance label of $u$ by $\FTDistLabel(u)$. 

%Let $\mathcal{T}=\bigcup_{i=1}^{K}\TreeCover_i$ be the collection of tree covers with $K=O(\log (nW))$ scales of distances. We call an edge $(u,v)$ a \emph{tree edge} if it appears on at least one of trees in $\mathcal{T}$. Our routing schemes will be based on assigning labeling information for the tree edges. For a non-tree edge, it will be sufficient to obtain the extended ID of the edge that contains $O(\log n)$ bits. As we will see, these IDs would not be stored explicitly in the routing tables.  
%
%For every $i \in [1,K]$ for $K=\lceil \log(nW) \rceil$, let Let $H_i$ be set of heavy edges in $G$ of weight at least $2^i$, and define the $i^{th}$ tree-cover by $\TreeCover_i=\TreeCover(G\setminus H_i,\omega, 2^i,2k)$. 
%Let $\mathcal{T}=\bigcup \TreeCover_i$, and denote the tree edges by $E_T=\bigcup_{T_{i,j} \in \TreeCover_i} E(T_{i,j})$. Note that by Def. \ref{def:tree-cover}, $|E_T|=O(k n^{1+1/(2k)} \log(nW))$. 
%

\mtodo{Added the part from here. This adds port and tree routing information to the ids, and adapts Lemma \ref{lem:useful-recovery-edges} (finding succinct path description) to the context of routing.}

%\mtext{
We slightly modify the connectivity label of the edges and vertices by augmenting them with routing information. 
Specifically, we define the vertex identifier $\ID_T(u)=[\ID(u), L_T(u)]$ where $L_T(u)$ is taken from Fact \ref{fc:route-trees}. We then slightly modify the 
the connectivity label of Eq. (\ref{{eq:conn-node}}) by defining 
$$\FTConnLabel_{G,T}(u)=\langle \LCALabel_T(u), \ID_T(u) \rangle~.$$
In addition, we also augment the extended identifier of an edge Eq. (\ref{eq:extend-ID}) with port information and tree routing information, by having:
$$\EID(e)=[\UID(e), \ID(u), \ID(v), \LCALabel_T(u), \LCALabel_T(v), \port(u,v), \port(v,u), L_T(u), L_T(v)]~,$$
where $\port(u,v)$ is the port number of the edge $(u,v)$ for $u$. 
%
%
%We next discuss a variant of Lemma \ref{lem:useful-recovery-edges} that is useful in the context of routing. 
%We use the following notation. For a vertex $v$, and a tree $T$ where $v \in T$, let $ID_T(v)=(\LCALabel(v),L_T(v))$, where $\LCALabel_T(v)$ is the ancestry label of $v$ in the tree $T$. For an edge $e=(u,v)$ where $u,v \in T$, we define the extended identifier $ID_T(e)$ as follows. $ID_T(e)$ is defined as in Section \ref{sec:ftconn-sketch}, but we also add to it port information and tree routing information. 
%
%
%
%First, we add to the extended identifier $ID_T(e)$ the port number of $v$ w.r.t $u$ and vice-versa. In addition, we add to $ID_T(e)$ the tree routing labels $L_T(u),L_T(v)$ from Fact \ref{fc:route-trees}. Note that the size of the ids is still $O(\log{n})$. 
Throughout this section, when applying the connectivity labels from Section \ref{sec:ftconn-sketch} on a graph $G$ with spanning tree $T$, we use these labels and extended identifiers to support routing.
%First, to support routing, when we apply the connectivity labels from Section \ref{sec:ftconn-sketch} on a graph $G$ with spanning tree $T$, we add to the identifiers $ID(e)$ port information and tree routing information. For each edge $e=(u,v)$, we add to the extended identifier $ID(e)$ the port number of $v$ w.r.t $u$ and vice-versa. In addition, we add to $ID(e)$ the tree routing labels $L_T(u),L_T(v)$ from Fact \ref{fc:route-trees}. Note that the size of the ids is still $O(\log{n})$. We also add to the connectivity label of a vertex $v$, its tree routing label $L_T(v)$. 
We later apply the connectivity labels with respect to the different trees of the tree cover as discussed in Section \ref{sec:ft-distance}. 
Let $T_{i,j} \in \TreeCover_i$, recall that $G_{i,j}=G[V(T_{i,j})]$ and that $\mathcal{T}=\bigcup_{i=1}^K \TreeCover_i$ for $K=O(\log (nW))$. 
%Recall that for a vertex $t$, the graph $G_{i,i^*(t)}$ contains the $2^i$ ball of $t$ in $G$, where $ T_{i,i^*(t)}$ is the corresponding tree from the tree cover that spans $G_{i,i^*(t)}$. We denote $G_i = G_{i,i^*(t)}, T_i = T_{i,i^*(t)}$. Using Lemma \ref{lem:useful-recovery-edges} ,we have the following.

\begin{lemma}\label{lem:succint_path_routing}
Consider a triplet $s,t,F$ such that $s,t,F \in G_{i,j}$. 
Given $ID_{T_{i,j}}(s),ID_{T_{i,j}}(t)$ and the connectivity labels $\{\FTConnLabel_{G_{i,j},T_{i,j}}(e)\}_{e \in F}$, we can determine w.h.p if $s$ and $t$ are connected in $G_{i,j} \setminus F$. If they are connected, we can output a labeled $s$-$t$ path $\widehat{P}$ of length $O(f)$ that provides a succinct description of the $s$-$t$ path in $G_{i,j} \setminus F$. The edges of $\widehat{P}$ are labeled by $0$ and $1$, where $0$-labeled edges correspond to $G_{i,j}$-edges and $1$-labeled edges $e=(x,y)$ correspond to $x$-$y$ paths in $T_{i,j} \setminus F$. For each $G_{i,j}$-edge, the succinct path description has the port information of the edge, and for each $x-y$ path, the description has the tree routing labels $L_{T_{i,j}}(x),L_{T_{i,j}}(y)$.
The length of the $s$-$t$ path encoded by $\widehat{P}$ is bounded by $(4k-1)(f+1)\cdot 2^i$. 
\end{lemma}

\mtodo{For the proof I use the fact that the decoding algorithm only uses the ancestry labels of $s,t$, we should probably add some remark on the topic also on the labels section.}

\begin{proof}
The proof follows the proof of Lemma \ref{lem:useful-recovery-edges}. To see this, first note that the decoding algorithm from Section \ref{sec:ftconn-sketch} mostly uses the connectivity labels of the faulty edges $F$, and it needs only the labels $\LCALabel(s),\LCALabel(t)$ of $s$ and $t$, to detect the connected components of $s$ and $t$ in $T_{i,j} \setminus F$. \mtodo{do we want to edit this there? at least have some remark} 
Hence, using $ID_{T_{i,j}}(s),ID_{T_{i,j}}(t)$ and the connectivity labels $\{\FTConnLabel_{G_{i,j},T_{i,j}}(e)\}_{e \in F}$, we can first check if $s$ and $t$ are connected in $G_{i,j} \setminus F$ using the decoding algorithm of Section \ref{sec:ftconn-sketch}. If they are connected, then from Lemma \ref{lem:useful-recovery-edges}, we get a succinct description of the $s$-$t$ path in $G_{i,j} \setminus F$. We next show that the algorithm indeed has the relevant port and tree routing information. For this note that all the vertices in the path $\widehat{P}$ obtained by Lemma \ref{lem:useful-recovery-edges} are either $s$ and $t$ or endpoints of the $f$ recovery edges found in the algorithm. The ids $ID_{T_{i,j}}(s),ID_{T_{i,j}}(t)$ of $s$ and $t$ have their tree routing information, and when the algorithm finds a recovery edge, it learns about its extended id $ID_{T_{i,j}}(e)$ that has the port information and tree routing information of its endpoints. Any $G_{i,j}$-edge in $\widehat{P}$ is a recovery edge, hence the algorithm has its port information, and for any $x$-$y$ path in $T_{i,j} \setminus F$, the algorithm has the tree routing labels $L_{T_{i,j}}(x),L_{T_{i,j}}(y)$, as needed.
The stretch analysis follows the stretch analysis in Section \ref{sec:ft-distance}. It is based on the fact that $\widehat{P}$ has as most $f+1$ subpaths in $T_{i,j} \setminus F$, each of length at most $(4k-2)2^i$, and at most $f$ recovery edges of weight at most $2^i$.
\end{proof}
%}







\subsection{Forbidden Set Routing (Faulty Edges are Known)}\label{sec:routing-known}
We start by describing the routing scheme in the forbidden set setting, where the faulty edges $F$ are known to the source vertex $s$. We show the following.

\begin{theorem}\label{thm:routing-known}[Forbidden-Set Routing]
For every integers $k,f$, there exists an $f$-sensitive compact routing scheme that given a message $M$ at the source vertex $s$, a label of the destination $t$, and labels of at most $f$ forbidden edges $F$ (known to $s$), routes $M$ from $s$ to $t$ in a distributed manner over a path of length at most $(8k-2)(f+1)\cdot \dist_{G \setminus F}(s,t)$. The table size of each vertex is bounded by $\widetilde{O}(n^{1/k} \log{(nW)})$. The header size of the messages is bounded by $\widetilde{O}(f)$ bits. The labels of vertices and edges have size $\widetilde{O}(n^{1/k} \log{(nW)})$.
\end{theorem}

\mtodo{I edited a bit the proof so it's more similar to the next section and uses Lemma \ref{lem:succint_path_routing}. The routing tables here still use the distance labels. Also, added a bit more details on the routing process.}

\begin{proof}
The algorithm is based on the distance labels from Section \ref{sec:ft-distance}. Recall that the distance labels are based on applying fault tolerant connectivity labels on different graphs $G_{i,j}$, we use the connectivity labels from Section \ref{sec:ftconn-sketch}.
The routing table of each vertex $u$ consists of its distance label and the tree routing labels from Fact \ref{fc:route-trees} for every tree $T_{i,j} \in \mathcal{T}$ containing $u$. That is,
$$R_{route}(u)=\FTDistLabel(u) \cup \{ \langle L_{T_{i,j}}(u), (i,j) \rangle ~\mid~ i \in [1,K], j \in \{1,\ldots, |\TreeCover_{i}|\}, u \in T_{i,j}\}~.$$
Since each vertex $u$ participates in $O(k n^{1/k} \log(n W))$ trees of $\mathcal{T}$, and since the distance labels are of size $O(k n^{1/k} \log(n W) \cdot \log^3{n})$, the table $R_{route}(u)$ has $O(k n^{1/k} \log(n W) \cdot \log^3{n})$ bits.
The label of a vertex $u$ is just $R_{route}(u)$, and the label of an edge $e$ is $\FTDistLabel(e)$. The labels have size $O(k n^{1/k} \log(n W) \cdot \log^3{n})$. \mtodo{we can have shorter labels for vertices as in the next section (but then we need to "open the box" of the distance labels), as the labels of edges are anyway large I'm not sure if we want to do it in this section.}

\mtext{
In the routing algorithm, the vertex $s$ is given the label $R_{route}(t)$ of $t$, and the labels $\{\FTDistLabel(e)\}_{e \in F}$, and it needs to route a message to $t$ in the graph $G \setminus F$. First, from the distance labels of $s,t$ and $F$, $s$ can check using the algorithm from Section \ref{sec:ft-distance} if $s$ and $t$ are connected in $G \setminus F$, and if so get a succinct description of a path between them. In more detail, recall that the algorithm from Section \ref{sec:ft-distance} works in $K$ phases, where in phase $i$ it checks if $s$ and $t$ are connected in the graph $G_{i,i^*(s)} \setminus F$ that contains the $2^i$-ball around $s$. Let $i$ be the first iteration where $s$ and $t$ are connected in $G_{i,i^*(s)} \setminus F$ according to the algorithm, and denote $G_i = G_{i,i^*(s)},T_i = T_{i,i^*(s)}$, and let $F_i = F \cap G_i$. The algorithm can also give a succinct description of an $s$-$t$ path in $G_i \setminus F_i$ following Lemma \ref{lem:succint_path_routing}. For this, note that we indeed have all the required information. The distance labels of edges in $F$ in particular contain the labels $\{\FTConnLabel_{G_i,T_i}(e)\}_{e \in F_i}$, and we can also tell which edges of $F$ are in $G_i$ from the labels. Also, the labels of $s,t$ contain the information $ID_{T_i}(s),ID_{T_i}(t)$ if they are both in $T_i$ (otherwise, they are not connected in level $i$).

The path $\widehat{P}$ as described in Lemma \ref{lem:succint_path_routing} is composed of $O(f)$ parts, where segment $(x,y)$ in the path corresponds either to an edge in $G_i$ or to a tree path in $T_i \setminus F$, it also has the relevant port and tree routing information. Our goal is to route a message according to this path. For this we add to the header of the message the description of $\widehat{P}$, the indexes $(i,i^*(s))$ of the tree we explore and an index $1 \leq q \leq 2f+1$ that represents the segment of $\widehat{P}$ we currently explore, initially $q=1$. Overall, the header size is $\widetilde{O}(f)$. To route a message according to the path, we work as follows. The header specifies the current segment in $\widehat{P}$. If the current segment corresponds to an edge $(x,y) \in G$, then $x$ uses the port information to route the message to $y$ and increases the index $q$. Otherwise, the current segment represents a tree path $(x,y) \in T_i$ and a vertex $u$ in this path uses its routing label in $T_i$ and the routing label of $y$ in $T_i$ (that is part of the header) to route the message towards $y$. When the message reaches $y$, it increases the index $q$. This completes the description of the routing process. The length of the path described is at most $(8k-2)(f+1)\cdot \dist_{G\setminus F}(s,t)$, as shown in Section  \ref{sec:ft-distance}. } 
%Given the labels $\{\FTDistLabel(w), w \in \{s,t\} \cup F\}$, the decoding algorithm of Lemma \ref{lem:approx-dist-recovery} computes a succinct description of an $s$-$t$ path in $G \setminus F$ of length $(8k-2)(f+1)\cdot \dist_{G\setminus F}(s,t)$. This description is given by a path $\widehat{P}$ augmented with the index $(i,j)$, such that every non-$G$ edge $e'=(u,v)$ of $\widehat{P}$ corresponds to a $u$-$v$ path in $T_{i,j}\setminus F$. Our routing scheme augments each vertex $v$ on $\widehat{P}$ with its tree label $L_{T_{i,j}}(v)$ from Fact \ref{fc:route-trees}. Overall, this information is encoded in $O(f\log^2 n)$ \mtodo{why $\log^2 n$?} bits which are attached to the header of the message. As each $G$-edge on $\widehat{P}$ is augmented with the port information, and each non-$G$ edge $(u,v)$ is augmented with the tree labels of $u,v$ in $T_{i,j}$, the vertices have the required information to route the message along the $s$-$t$ path encoded by $\widehat{P}$. 
\end{proof}

%We therefore have:
%\begin{enumerate}[noitemsep]
%\item }.
%\item Every non-$G$ edge $e=(u,v)$ corresponds to a tree path $T \in \bigcup_i\TreeCover_i$
%\item The 
%\end{enumerate}


\subsection{Fault Tolerant Routing (Faulty Edges are Unknown)}\label{sec:route-unknown}
We now consider the more involved setting where the set of failed edges $F$ are unknown to $s$. In this case, an edge $(u,v) \in F$ is detected only when the message arrives, during the routing procedure, to one of the endpoints of $e$. Note that the routing scheme should, by definition, be prepared to any set of faulty edges $F$. However, the space bound of our scheme is required to be bounded by $\widetilde{O}(f n^{1+1/k})$, which is possibly much smaller than the number of graph edges $m$. This in particular implies that we cannot store the FT-distance labels of all the graph edges. Nevertheless, we show that it is sufficient to explicitly store the labeling information for the tree edges in $\mathcal{T}$. The required information for the failed non-tree edges would be revealed throughout the process, by applying the decoding algorithm of Lemma \ref{lem:succint_path_routing}.
Our routing scheme eventually routes the message along the $s$-$t$ path encoded by the FT-distance labels of $s,t$ and $F$. However, since the labels of $F$ are unknown in advance, the routing scheme will detect these edges in a trail and error fashion which induces to an extra factor of $f$ in the final multiplicative stretch. This extra $f$ factor is also shown to be essential, in the end of the section.
We proceed by describing the routing tables.  
%A routing scheme consists of a two phases algorithm. In the preprocessing phase, each vertex $v$ is assigned
%a routing table $R(v)$ and a label $L(v)$. In the routing phase, a vertex $u$ gets a message with a short header
%$H(M)$ and with a destination label $L(v)$, and based on its own routing table $R(u)$, the destination label $L(v)$
%and the header $H(M)$, it decides to which neighbor $w$ to forward the message. It can also add information to the header of the message. The key objective is to minimize the individual size of each label $L(u)$, routing tables $R(u)$ and the message header $H(M)$. 

\remove{
\paragraph{The routing tables.} For ease of presentation, we first describe a solution with a multiplicative stretch of $O(kf^2)$, and \emph{global} space of $\widetilde{O}(f K \cdot n^{1+1/k})$, \mtodo{should it be $n^{1+2/k}$?} but the individual tables of some of the vertices might be of linear space. 
Recall that $\mathcal{T}=\bigcup_i^{K} \TreeCover_i$, for $K=O(\log (nW))$ is a collection of tree covers in all $K=\lceil \log (nW) \rceil$ distance scales, see Eq. (\ref{eq:TC-i}). For every vertex $u$, let $\deg_T(u)=\sum_{T_{i,j} \in \mathcal{T}}\deg(u,T_{i,j})$ be the sum of degrees of $u$ in the collection of trees  $\mathcal{T}$.
The algorithm computes each vertex $u$ a table of $\widetilde{O}(f \cdot \deg_T(u) \cdot n^{1/k})$ bits.
Since the total number of tree edges in $\mathcal{T}$ is bounded by $\widetilde{O}(K \cdot n^{1+1/k})$, this provides a global space bound of $\widetilde{O}(fK \cdot n^{1+2/k})$ bits. We later on improve the space of each table to $\widetilde{O}(fK \cdot n^{2/k})$ bits. \mtodo{maybe extra $k,K$ are needed in some places.}

The routing process has at most $f+1$ phases, and each phase uses an independent set of randomized FT-distance labels. Therefore, the preprocessing algorithm employs $f$ \mtodo{$f$ or $f+1$?} independent applications of the $(f,(8k-2)(f+1))$ FT-distance labels scheme. Denote the output labels obtained by the $i^{th}$ application by $\FTDistLabel_i(w)$ for every $w \in V(G)\cup E(G)$. Let $E_T=\bigcup_{T_{i,j} \in \mathcal{T}} E(T_{i,j})$ be the collection of tree edges. The \emph{routing label} \mtodo{maybe we want to have shorter labels, and have this information only in the routing tables?} of each $w \in V\cup E_T$ is given by 
$$L_{route}(w)=\{\FTDistLabel_1(w),\ldots, \FTDistLabel_{f+1}(w)\}~.$$ 
The routing label $L_{route}(e)$ of a non-tree edge $e \in E \setminus E_T$ is simply the extended identifier of $e$. For each vertex $u$, the routing table $R_{route}(u)$ consists of the following:
\begin{enumerate}%[noitemsep]
\item Tree labels $L_{T_{i,j}}(u)$ for every tree $T_{i,j}$ in $\mathcal{T}$ that contains $u$ (from Fact \ref{fc:route-trees}). These labels are augmented with their corresponding tree index $(i,j)$.
\item The routing labels $L_{route}(u)$ and $\{L_{route}(e=(u,v)) ~\mid~ e \in T_{i,j}, T_{i,j} \in \mathcal{T}\}$.
\end{enumerate}
The header information initially contains the succinct path information\footnote{\textbf{MP: This is not essential, we can always make the header contain the labels of the currently detected faults.}} obtained by the decoding algorithm of the FT-distance labeling when given the labels $L_{route}$ of $s$ and $t$. \mtodo{do we want to have $f$ paths? Or only one of them that is relevant for the current phase}  As we will see, throughout the routing procedure, the header information will be augmented with the labels of the currently detected faulty edges. 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{The routing tables.} For ease of presentation, we first describe a solution with a multiplicative stretch of $O(kf^2)$, and \emph{global} space of $\widetilde{O}(f K \cdot n^{1+1/k})$, but the individual tables of some of the vertices might be large. We later on improve the space of each table to $\widetilde{O}(fK \cdot n^{1/k})$ bits.

Recall that $\mathcal{T}=\bigcup_i^{K} \TreeCover_i$, for $K=O(\log (nW))$ is a collection of tree covers in all $K=\lceil \log (nW) \rceil$ distance scales, see Eq. (\ref{eq:TC-i}). For every vertex $v$, let $\deg_T(v)=\sum_{T_{i,j} \in \mathcal{T}}\deg(u,T_{i,j})$ be the sum of degrees of $u$ in the collection of trees  $\mathcal{T}$. Recall that $G_{i,j}=G[V(T_{i,j})]$.
\mtext{For the routing we apply the FT-connectivity labels on the graphs $G_{i,j}$, similarly to Section \ref{sec:ft-distance}.
The routing process uses $f$ independent applications of randomized FT-connectivity labels from Section \ref{sec:ftconn-sketch}, applied on each one of the graphs $G_{i,j}$. \mtodo{There is some delicate issue here. In my understanding we do want to have the extended ids fixed in different applications, and only change the randomness of sketches, as I try to explain here.} In more detail, when we apply the labeling scheme on the graph $G_{i,j}$ with spanning tree $T_{i,j}$, we use $f$ independent random seeds $\mathcal{S}_h$ to determine the randomness of the sketches. However, the seed $\mathcal{S}_{ID}$ used to determine the extended ids of edges in $G_{i,j}$ is fixed in the $f$ applications, hence the ids are fixed and we only use fresh randomness to compute the sketch information. This process is done independently on each one of the graphs $G_{i,j}$. }  
Denote the output labels obtained by the ${\ell}^{th}$ application of the scheme on the graph $G_{i,j}$ by $\FTConnLabel^{\ell}_{G_{i,j},T_{i,j}}(w)$ for every $w \in V(G_{i,j})\cup E(G_{i,j})$, and we denote by $$\FTConnLabel_{G_{i,j},T_{i,j}}(w)=(\FTConnLabel^1_{G_{i,j},T_{i,j}}(w),...,\FTConnLabel^f_{G_{i,j},T_{i,j}}(w)).$$
Since in each application the labels are of size $O(\log^3{n})$, the total size of each label is $O(f \log^3{n})$. \mtext{Recall that for a non-tree edge $e \in G_{i,j}$, we have that  $\FTConnLabel^{\ell}_{G_{i,j},T_{i,j}}(e)=\ID_{T_{i,j}}(e)$. This label does not depend on the sketch information, and hence is the same in all $f$ applications, we will exploit this later in the algorithm.}

\mtodo{I changed a bit the definition of routing tables and labels. The labels currently are of polylog size (no extra $f$ or $n^{1/k}$).}
\mtext{
The routing table $R_{route}(v)$ of a vertex $v$ has the following information for any tree $T_{i,j}$ such that $v \in T_{i,j}$:
\begin{enumerate}
\item The values $(ID_{T_{i,j}}(v),i,j)$.
\item The connectivity labels $\FTConnLabel_{G_{i,j},T_{i,j}}(e)$ for any tree edge $e \in T_{i,j}$ adjacent to $v$. 
\end{enumerate}

Since the connectivity labels are of size $\widetilde{O}(f)$, and since $v$ appears in $\deg_T(v)$ trees, the size of the table is $\widetilde{O}(f \deg_T(v)).$ Since the total number of tree edges in $\mathcal{T}$ is bounded by $\widetilde{O}(K \cdot n^{1+1/k})$, this provides a global space bound of $\widetilde{O}(fK \cdot n^{1+1/k})$ bits.

Recall that for a vertex $v$ and index $1 \leq i \leq K$, we denote by $i^*(v)$ an index such that the $2^i$-ball around $v$ is contained in $T_{i,i^*(v)}$.
The routing label $L_{route}(v)$ of $v$ has the id of $v$ in the trees $T_{i,i^*(v)}$.
$$L_{route}(v) = \{(i^*(v),ID_{T_{i,i^*(v)}}(v)) | i \in [1,K]\}$$

The size of the label is $O(K\log{n})=O(\log{n} \log{nW})$.}

\mtodo{In the routing algorithm the main difference is that we have log iterations for the different trees, in each tree the algorithm is similar to before.}

\paragraph{The routing algorithm.} \mtext{In the routing algorithm, the source vertex $s$ gets the routing label $L_{route}(t)$ of the destination $t$ and its goal is to find a graph $G_{i,j}$ such that $s$ and $t$ are connected in $G_{i,j} \setminus F$, and use it for routing. As the set $F$ is not known in advance, the algorithm works in $K= O(\log{nW})$ iterations, where in iteration $i$ it tries to route a message in $G_{i,i^*(t)}$. If $s$ and $t$ are connected in $G_{i,i^*(t)} \setminus F$ the algorithm succeeds, and otherwise we proceed to the next iteration. 
We next describe the algorithm for one iteration $i$, we denote $G_i = G_{i,i^*(t)}, T_i = T_{i,i^*(t)}$. Note that $s$ learns the index $i^*(t)$ from the label of $t$, and it can check if $s \in T_i$ using its routing table. If $s \not \in T_i$, we proceed to the next iteration.}

If $s \in T_i$, the routing procedure for iteration $i$ has at most $f+1$ phases. Each phase will start at the source vertex $s$. We will maintain the following invariant in the beginning of each phase $\ell \in \{1,\ldots, f+1\}$: (i) the algorithm has already detected a subset of $\ell-1$ faulty edges $F_\ell \subseteq F$, and (ii) the header contains the labels $\FTConnLabel_{G_i,T_i}(e)$ of all the edges $e \in F_\ell$. Each phase $\ell \leq f+1$ will terminate either at the destination vertex $t$, or at the source vertex $s$. In addition, w.h.p., if $s$ and $t$ are connected in $G_i \setminus F$, phase $f+1$ will terminate at $t$. The invariant holds vacuously for phase $1$.

We now describe the $\ell^{th}$ phase of the routing procedure given the invariant. The source vertex $s$ considers the $\ell^{th}$ copy of the FT-connectivity labels, $\FTConnLabel^{\ell}_{G_i,T_i}(e)$ for every $e \in F_\ell$. 
Using the connectivity labels, that are part of the header, and the ids $ID_{T_i}(s),ID_{T_i}(t)$ that are part of the routing table of $s$ and routing label of $t$, the algorithm first checks if $s$ and $t$ are connected in $G_i \setminus F_\ell$ using Lemma \ref{lem:succint_path_routing}. If the answer is no, the algorithm moves to the next iteration $i+1$.
Otherwise, by applying the decoding algorithm of Lemma \ref{lem:succint_path_routing}, it computes the succinct path $\widehat{P}_\ell$. The path $\widehat{P}_\ell$ encodes an $s$-$t$ path in $G_i \setminus F_\ell$, that includes the relevant port and tree routing information of its vertices. The header of the message $H_\ell$ then contains 
$$H_\ell=\langle \widehat{P}_\ell, i, i^*(t), \{\FTConnLabel_{G_i,T_i}(e)\}_{e \in F_{\ell}}, q \rangle~,$$ where $q = O(f)$ is an index indicating the current segment of $\widehat{P}_\ell$ we explore. \mertodo{$H_\ell$ should contain $\FTConnLabel^{\ell}_{G_i,T_i}(e)$, right?}


\mtext{The size of the header is $\widetilde{O}(f^2)$, as the description of the path has size $\widetilde{O}(f)$, and additionally we have at most $f$ faulty edges with labels of size $\widetilde{O}(f)$.} \mtodo{in some sense we don't really need to have all this $O(f^2)$ information on the header at once because it's enough that $s$ learns in each phase on one of the labels and then stores it locally, but this I guess doesn't work with the formal definition of routing.}
Let $P_\ell$ be the $G$-path encoded by the path $\mathcal{P}_\ell$. The algorithm then routes the message along $P_\ell$ in the same manner as in Sec. \ref{sec:routing-known}. In the case where $P_{\ell}\cap F=\emptyset$, the phase successfully terminates at the destination vertex $t$. From now on, we consider the case that $P_{\ell}$ contains at least one faulty edge. 

Let $e=(u,v)$ be the first edge (closest to $s$) on the path $P_\ell$ that belongs to $F$. Since $P_\ell \cap F_\ell=\emptyset$, it holds that $e \in F \setminus F_\ell$. Without loss of generality, assume that $u$ is closer to $s$ on $P_\ell$. Thus the faulty edge $e$ is detected upon arriving to the vertex $u$. 
In the case where $e$ is a \emph{non-tree edge}, then it must be a $G$-edge on $\widehat{P}_\ell$. Since this path has the ids $ID_{T_i}(e)$ of its $G$-edges, and since the connectivity label of a non-tree edge $e$ is $ID_{T_i}(e)$ in all the $f$ applications of the scheme on $G_i$, $u$ can add $\FTConnLabel_{G_i,T_i}(e)$ to the header of the message. \mtodo{here we use the fact that the extended ids are the same in all $f$ phases (of the same tree)} Assume now that $e$ is a tree edge in $T_i$. The vertex $u$ then adds the label $\FTConnLabel_{G_i,T_i}(e)$ to the header of the message, as $e$ is a tree edge adjacent to $u$ it has this information in its routing table. Finally, it marks the header with the sign $R$, indicating that the message should now be routed in the reverse direction, until arriving $s$ again. This completes the description of phase $\ell$. It is easy to see that the invariant is maintained. If $s$ and $t$ are connected in $G_i \setminus F$, after at most $f$ phases all faulty edges are detected. In the last phase, the path computed based on the labeling information is free from faulty edges, and the routing is completed (in the same manner as in Sec. \ref{sec:routing-known}) at the destination $t$. We next bound the multiplicative stretch of the routing.

%The routing procedure has at most $f+1$ phases. Each phase will start at the source vertex $s$. We will maintain the following invariant in the beginning of each phase $\ell \in \{1,\ldots, f+1\}$: (i) the algorithm has already detected a subset of $\ell-1$ faulty edges $F_\ell \subseteq F$, and (ii) the header contains the labels $L_{route}(e)$ of all the edges $e \in F_\ell$. \mtodo{what happens with edges that are non-tree edges in some of the trees and tree edges in some later trees? Not sure that we learn the relevant information about it, maybe need to find it again?} Each phase $\ell \leq f$ will terminate either at the destination vertex $t$, or at the source vertex $s$. In addition, w.h.p., phase $f+1$ will terminate at $t$. \mtodo{if there is a path to $t$?}  The invariant holds vacuously for phase $1$. 

%We now describe the $\ell^{th}$ phase of the routing procedure given the invariant. The source vertex $s$ considers the $\ell^{th}$ copy of the FT-distance labels, $\FTDistLabel_\ell(w)$ for every $w \in \{s,t\} \cup F_\ell$. 
%By applying the decoding algorithm of Lemma \ref{lem:approx-dist-recovery}, it computes the succinct path $\widehat{P}_\ell$ along with a tree index $(i_\ell,j_\ell)$. The path $\widehat{P}_\ell$ encodes an $s$-$t$ path in $G[V(T_{(i_\ell,j_\ell)})] \setminus F_\ell$.  As in the previous section, the source $s$ augments this path with the tree labels (of Fact \ref{fc:route-trees}) of the vertices on $\mathcal{P}$. The header of the message $H_\ell$ then contains 
%$$H_\ell=\langle \widehat{P}_\ell, (i_\ell,j_\ell), \bigcup_{v \in \widehat{P}_\ell} L_{T_{i_\ell,j_\ell}}(v) \rangle~.$$
%Let $P_\ell$ be the $G$-path encoded by the path $\mathcal{P}_\ell$. The algorithm then routes the message along $P_\ell$ in the same manner as in %Sec. \ref{sec:routing-known}. In the case where $P_{\ell}\cap F=\emptyset$, the phase successfully terminates at the destination vertex $t$. From now on, we consider the case that $P_{\ell}$ contains at least one faulty edge. 

%Let $e=(u,v)$ be the first edge (closest to $s$) on the path $P_\ell$ that belongs to $F$. Since $P_\ell \cap F_\ell=\emptyset$, it holds that $e \in F \setminus F_\ell$. Without loss of generality, assume that $u$ is closer to $s$ on $P_\ell$. Thus the faulty edge $e$ is detected upon arriving to the vertex $u$. 
%In the case where $e$ is a \emph{non-tree edge}, then it must be a $G$-edge on $\widehat{P}_\ell$. Since this path is augmented with the extended ID of its $G$-edges, $u$ can add the extended ID of $e$ to the header of the message.  Assume now that $e$ is a tree edge, i.e., $e \in E_T$.  Specifically, by Lemma \ref{lem:approx-dist-recovery}, $e$ is an edge in the tree $T_{i_\ell,j_\ell}$. The vertex $u$ then adds the label $L_{route}(e)$ \mtodo{if we add the complete label, it makes the headers large} to the header of the message. Finally, it marks the header with the sign $R$, indicating that the message should now be routed in the reverse direction, until arriving $s$ again.  This completes the description of phase $\ell$. It is easy to see that the invariant is maintained, and thus after at most $f$ phases all faulty edges are detected. In the latter case, the path computed based on the labeling information is free from faulty edges, and the routing is completed (in the same manner as in Sec. \ref{sec:routing-known}) at the destination $t$. We next bound the multiplicative stretch of the routing.

\mtodo{updated the stretch analysis.}

\mtext{
\begin{claim}\label{cl:route-length}
Fix a set of faulty edges $F$, and let $s,t$ be vertices that are connected in $G \setminus F$. Then, the message is routed from $s$ to $t$ within $32k (f+1)^2 \cdot \dist_{G \setminus F}(s,t)$ steps, w.h.p.
\end{claim}
\begin{proof}
First note that since each phase and each graph $G_{i}$ uses an independent set of FT-connectivity labels, then in each iteration and each phase the decoding algorithm succeeds w.h.p. and outputs an $s$-$t$ path $\widehat{P}_\ell$ if exists. 

Assume that $\dist_{G \setminus F}(s,t) \in (2^{i-1},2^i]$. Then, $s$ and $t$ are connected in $G_i \setminus F$, as $T_i = T_{i,i^*(t)}$ contains the $2^i$-ball around $t$. We show that the algorithm terminates at $t$ in iteration $i$ or before it, and that in any iteration $j \leq i$, the routing algorithm traverses a path of length at most $2(4k-1)(f+1)^2 \cdot 2^j$.

Let $j \leq i$. In the $\ell$'th phase of iteration $j$, the algorithm first checks if $s$ and $t$ are connected in $G_j \setminus F_{\ell}$, where $F_{\ell}$ is the set of currently detected faults. If the answer is no, the algorithm proceeds to the next iteration. Otherwise, it tries to route a message from $s$ to $t$ on the path encoded by $\widehat{P}_{\ell}$. The length of the path is bounded by $(4k-1)(f+1)\cdot 2^j$ from Lemma \ref{lem:succint_path_routing}. The algorithm either succeeds, or finds a faulty edge on the way in which case it returns to $s$ by traversing the same path on the reverse direction. Overall, the algorithm traverses a path of length at most $2(4k-1)(f+1)\cdot 2^j$, in this phase. In all $f+1$ phases of iteration $j$, the length of the path explored is at most $2(4k-1)(f+1)^2 \cdot 2^j$. Summing over all iterations $j \leq i$, the stretch is bounded by $$\sum_{j=1}^{i} 2(4k-1)(f+1)^2 \cdot 2^j = 2(4k-1)(f+1)^2 \sum_{j=1}^i 2^j \leq 2^{i+2} (4k-1)(f+1)^2 \leq 32k (f+1)^2 \dist_{G \setminus F}(s,t).$$ The last inequality uses the fact that $2^{i-1} \leq \dist_{G \setminus F}(s,t).$ 

In the $i$'th iteration, since $s$ and $t$ are connected in $G_i \setminus F$, then for any $F_{\ell} \subseteq F$, $s$ and $t$ are connected in $G_i \setminus F_{\ell}$, hence the algorithm always finds a path $\widehat{P}_{\ell}$. Hence, it either succeeds in routing the message to $t$ in one of the phases (or one of the previous iterations), or learns about all the failures $F$. In the latter case, in phase $f+1$ it learns about a failure-free path $\widehat{P}_{f+1}$, and the routing terminates at $t$. This completes the proof.
\end{proof}
}

\remove{
\begin{claim}\label{cl:route-length}
Fix a set of faulty edges $F$. Then, the message is routed from $s$ to $t$ within $(16k-4)(f+1) f\cdot \dist_{G \setminus F}(s,t)$ steps, w.h.p.
\end{claim}
\begin{proof}
First note that since each phase and each graph $G_{i}$ uses an independent set of FT-connectivity labels, w.h.p., the decoding algorithm of phase $\ell$ applied on the label set $\{\FTDistLabel(w), w \in \{s,t\} \cup F_\ell\}$ succeeds w.h.p. and outputs an $s$-$t$ path $\widehat{P}_\ell$. 

Let $P_{\ell}$ be the $s$-$t$ path in $G \setminus F_\ell$ encoded by $\widehat{P}_\ell$. By Lemma \ref{lem:approx-dist-recovery}, the length of $P_\ell$ is bounded by $(8k-2)(f+1)\cdot \dist_{G \setminus F_\ell}(s,t)$. Since in phase $\ell$ the message is routed along a (possibly) partial path $P_\ell$ and back to $s$, we have $2|P_\ell|$ routing hops \mtodo{change to capture weighted graphs?} in that phase. Overall, we have at most $2\sum_{i=1} |P_\ell|$ routing hops. Since 
$F_\ell \subseteq F$ for every $\ell$, it holds that $\dist_{G \setminus F_\ell}(s,t)\leq \dist_{G \setminus F}(s,t)$, and consequently $(16k-4)(f+1) f \cdot \dist_{G \setminus F}(s,t)$ routing steps over all. The claim follows. 
\end{proof}
}

To conclude, we have the following.

\begin{theorem}
For every integers $k,f$, there exists an $f$-sensitive compact routing scheme that given a message $M$ the source vertex $s$ and a label $L_{route}(t)$ of the destination $t$, in the presence of at most $f$ faulty edges $F$ (unknown to $s$) routes $M$ from $s$ to $t$ in a distributed manner over a path of length at most $32k (f+1)^2\cdot \dist_{G \setminus F}(s,t)$. 
The global table size is $\widetilde{O}(f \cdot n^{1+1/k} \log{(nW)})$.
The header size of the messages is bounded by $\widetilde{O}(f^2)$ bits, and the label size of vertices is $O(\log{(nW)} \log{n})$. 
\end{theorem}


 %$R_{T}(u)$ for every $T \in \TreeCover_i$ for $i \in \{1,\ldots, \log (nW)\}$. In addition, $u$ stores the $(f,k)$ FT-approximate labels of $u$ and each of its incident edges in $\mathcal{T}$. Let $\dist_{G \setminus F}(s,t) \in (2^i, 2^{i+1}]$ and let $T_{i,j}$ be a tree in $\TreeCover_i$ containing both $s$ and $t$.  Initially the scheme attempts to route the message from $s$ to $t$ using the edges of $T_{i,j}$ alone. Note that indeed all vertices on $T_{i,j}$ contain the routing table $R_{T_{i,j}}$. If none of the faulty edges are on $T_{i,j}$, then we are done as the depth of $T_{i,j}$ is at most $(2k-1) 2^{i+1}$. Now, assume otherwise and let $e_1=(x_1,y_1)$ be the first edge on the $s$-$t$ path on $T_{i,j}$ that belongs to $F$. W.l.o.g. assume that $x_1$ is the vertex that appears first on the $\pi(s,t,T_{i,j})$ path. Since $e_1$ is in $T_{i,j}$ the vertex $x_1$ contains the FT-connectivity label of the edge $e_1$ in $G_{i,j}$. 
%
%Using Lemma \ref{lem:useful-recovery-edges}, the vertex $x_1$ which holds the labels $\FTConnLabel(s), \FTConnLabel(t)$ and $\FTConnLabel(e_1)$ can compute the recovery edge $q_1=(a_1,b_1)$ such that $(T_{i,j} \setminus e_1)\cup \{q_1\}$ is a tree that restores the connectivity of $s$ and $t$ (if possible).  The vertex $x_1$ then adds to the header of the message the identity of $e_1$, the recovery edge $q_1$ and the connectivity label $\FTConnLabel_{G_{i,j}}(e_1)$. The message is then forward to $a_1$ over the tree $T_{i,j}$. If the tree path from $x_1$ to $a_1$ in $T_{i,j}$ does not contain any edge from $F$, then we proceed to routing the message along the recovery edge $q_1$. Otherwise, another faulty edge $e_2=(x_2,y_2) \in F$ is detected. The endpoint $x_2$ then holds the FT-connectivity label of $e_2$, namely, $\FTConnLabel_{G_{i,j}}(e_2)$, and in addition from the header of the message and the label of $t$ is has $\FTConnLabel_{G_{i,j}}(w)$ for $w \in \{e_1,s,t\}$. Thus, it can compute the recovery edges $q'_1$ and $q'_2$. The names of the recovery edges as well as the FT-connectivity label of $e_2$ are added to the header of the message. Note that throughout the process the recovery edges provided at some point are turned out to be faulty as well. In the latter case, we will use the fact that the decoding algorithm of 
%the FT-connectivity scheme only needs the edge labels of $F \cap T_{i,j}$ and the identifiers of the remaining edges in $F \setminus T_{i,j}$.
%This process continues until all the faulty edges are revealed. In this case, at some point, some vertex $w$ holds the FT-connectivity labels of all the faulty edges in $T_{i,j}$ as well as the labels of $s$ and $t$. This allows $w$ to compute the of recovery edges $Q$ that restores the $s$-$t$ connectivity on $T_{i,j}\setminus F$. In addition, the decoding algorithm also outputs a succinct path description that describes the ordering of the $Q$ edges on the tree path in $(T_{i,j}\setminus F) \cup Q$. 


\mtodo{I didn't change the next section, as some of the definitions of routing tables/labels changed, there are probably also changes here.}

\paragraph{Improving the size of the routing tables.} 
So far, we have described a routing scheme that consumes a total space of $\widetilde{O}(f\cdot n^{1+1/k}\log (nW))$ bits, and multiplicative stretch %\footnote{Alternatively, by scaling this can be written as space of $\widetilde{O}(f\cdot n^{1+2/k}\log (nW))$ bits and stretch of $32(f+1)^2 k$.} 
$32(f+1)^2 k$. We now explain the required modifications needed to providing routing tables with $\widetilde{O}(f^2\cdot n^{1/k})$ bits per vertex. The most space consuming information for a vertex $u$ is the connectivity labeling
information of the edges incident to $u$ in each of the trees $T_{i,j} \in \mathcal{T}$. As the degree of $u$ in some of the trees might be $\Theta(n)$, it leads to tables of linear size. To reduce the space of the individual tables, we apply a load balancing idea which distributes the labeling information incident to \emph{high}-degree vertices among their neighbors. 

Instead of storing the labeling information of $e=(u,v)$ at the routing tables of $u$ and $v$, we define 
for every tree $T \in \mathcal{T}$ and an edge $e=(u,v) \in T$, a subset $\Gamma_T(e)$ of vertices that store the connectivity labeling information of $e$ in $T$. We will make sure that the information on some vertex in $\Gamma_T(e)$ can be easily extracted in the routing procedure, and that each vertex stores the information for a small number of edges in each tree. Consider an edge $e=(u,v)$ in a tree $T$, and assume, without loss of generality, that $u$ is the parent of $v$ in the tree $T$. In the case where $\deg(u,T)\leq f+1$, we simply let $\Gamma_T(e)=\{u,v\}$. That is, the label of $e$ is stored by both endpoints of $e$ (as before). The interesting case is where $\deg(u,T)\geq f+2$, in which case, $u$ might not be able to store the label of $e$, and will assist its other children as follows.  Let $Child(u,T)=[v_1,\ldots, v_\ell]$ be the lexicographically ordered list of the children of $u$ in $T$.  The algorithm partitions $Child(u,T)$ into consecutive blocks of size $f+1$ (the last block might have $2f+1$ vertices). Letting $[v_{q,1}, \ldots, v_{q,f+1}] \subseteq Child(u,T)$ be the block containing $v$, define
$$\Gamma_T(e)=\{v_{q,1}, \ldots, v_{q,f+1}\}~.$$
Note that in particular, $v \in \Gamma_T(e)$. Thus, the label of $e$ is stored by $v$ and $\ell \in [f,2f-1]$ additional children on $u$ in $T$. 

We then modify the tree labels from Fact \ref{fc:route-trees} to contain the port information of $\Gamma_T(e)$. 
To do that, we re-define the identifier of an edge $e$ to include the port information of $\Gamma_T(e)$. Thus, the identifier of an edge has $O(f\log n)$ bits. Using Fact \ref{fc:route-trees}, we then have tree labels of $O(f\log n)$ such that given the labels of $u$ and $t$, the algorithm can compute the port information $\Gamma_T(e)$ where $e$ is the edge incident to $u$ on the $u$-$t$ tree path in $T$. We have:
\begin{claim}\label{cl:tree-label-port}


\end{claim}

In addition, we modify the routing tables of each vertex $v$, so that its includes the connectivity labels $\FTConnLabel_{G_{i,j},T_{i,j}}(e)$ for any tree edge $e \in T_{i,j}$ such that $v \in \Gamma_{T_{i,j}}(e)$ for every tree $T_{i,j} \in \mathcal{T}$. This should be compared with the solution of the previous subsection, where $v$'s table contained the information for all its incident edges in $T_{i,j}$. We therefore have:
\begin{claim}\label{cl:route-balance-table}
The size of each routing table $R_{route}(v)$ is bounded by $\widetilde{O}(f K n^{1/k})$ bits.
\end{claim}
\begin{proof}
For every tree $T_{i,j}$ containing $v$, $v$ stores that connectivity label of $\widetilde{O}(f)$ bits of all edges in the set $E(v,T_{i,j})=\{e \in T_{i,j} ~\mid~ v \Gamma_{T_{i,j}}(e)\}$. Note that $|E(v,T_{i,j})|\leq f$ as each vertex stores the label of its parent in the tree, $O(f)$ child edges, and $O(f)$ child edges of its parent in the tree. Since each $v$ participates in $\widetilde{O}(K n^{1/k})$ trees, overall its routing table has $\widetilde{O}(f K n^{1/k})$ bits, as required. 
\end{proof}

It remains to explain the required modifications for the routing procedure. Upon arriving to a vertex $u$ incident to a faulty \emph{tree} edge $e=(u,v)$ the procedure is as follows. The interesting case is where $e$ is a tree edge in some path $\pi(x,y,T_{i,j})$ where $(x,y)$ is an edge in the succinct path $\widehat{P}$ indicated on the header of the message. 
In this case, the tree routing algorithm applied at $u$ is given the tree labels $L_{T_{i,j}}(u)$ and $L_{T_{i,j}}(y)$ and output the port information of $\Gamma_{T_{i,j}}(e)$ for the edge $e=(u,v)$ that lies on the tree path $\pi(u,y, T_{i,j})$. Since there are at most $f$ edge faults, and $\Gamma_{T_{i,j}}(e)$ contains information on at least $f+1$ ports of $u$'s neighbors that contain the label of $e$, the vertex $u$ can access a non-faulty neighbor, say $w$, that has the label information of $e$. That vertex can then add the labeling information of $e$ to the header of the message, and the routing algorithm proceeds as before. 



%%First, we slightly modify the routing labels by applying  $f+1$ independent applications of the $(f,2k)$ FT-distance labeling scheme. That is, we increase the stretch parameter by a factor of $2$ to yield more succinct-distance labels with label size of $\widetilde{O}(n^{1/(2k)}\log(nW))$ bits. As before, we denote the output label obtained by the $i^{th}$ application of the $(f,2k)$ FT-distance labeling scheme by $\FTDistLabel_i(w)$ for every $w \in V(G)\cup E_T$. 
%%We have that $L_{route}(w)=\{\FTDistLabel_1(w),\ldots, \FTDistLabel_{f+1}(w)\}$  has $\widetilde{O}(f n^{1/(2k)}\log (nW))$ bits, for every $w \in V\cup E_T$. The label of a non-tree edge is given by its extended edge identifier, as before. 
%The routing labels are unchanged, and the routing tables are modified as follows. For every tree $T_{i,j}\in \mathcal{T}$ containing $u$ the algorithm computes a table $R_{route,i,j}(u)$ defined as follows. Let $v$ be the parent of $u$ and let $N_{i,j}(v)=[v_1,\ldots, v_\ell]$ be the lexicographically ordered list of the children of $v$ in $T_{i,j}$. 
%The table $R_{route,i,j}(u)$ contains the labels $L_{route}(u)$, $L_{route}((u,v))$, and the edge labels connecting $u$ to its (lexicographically) first $f+1$ children in $T_{i,j}$. In the case where $u$ has at least $f+1$ brothers, i.e., $\ell \geq f+1$, the algorithm stores in $R_{route,i,j}(u)$ the labels of at most $2f$ edges connecting a subset of its brothers to the parent $v$.  The goal of this step is to provide a load balancing over the labels of the edges incident to the parent $v$. To determine this edge set, the list $N_{i,j}(v)$ is partitioned into consecutive blocks of size $f+1$ (the last block might have $2f+1$ vertices). The vertices of the $k$'th block in $N_{i,j}(u)$ will store the $L_{route}(e)$ labels of all the child edges of that block. Letting 
%$[v_{q,1}, \ldots, v_{q,f+1}]$ be the block containing $u$, then $u$ stores the labels $L_{route}(e')$ for every $e' \in \{ (v_{q,1},v), \ldots, (v_{q,f+1},v)\}$. Note that the block size is set to be at least $f+1$, to guarantee that at least one child edge in each block is non-faulty. Overall, $R_{route}(u)=\bigcup_{T_{i,j} \in \mathcal{T} ~\mid~ u \in T_{i,j}} R_{route,i,j}(u)$. 
%%Consider a tree $T_{i,j} \in \mathcal{T}$ and a vertex $u \in T_{i,j}$ with at least $f+1$ children in $T_{i,j}$. The labels $L_{route}(e)$ of its child edges $e$\footnote{I.e., edges connecting $u$ to its children in $T_{i,j}$.} are distributed among the children of $u$ in $T_{i,j}$ as follows. 
%%Let $N_{i,j}(u)=\{v_1,\ldots, v_\ell\}$ be an ordered list of $u$'s children in the tree $T_{i,j}$. The algorithm partitions the neighbor set $N_{i,j}(u)$ into consecutive blocks of size $f+1$ (the last block might have $2f+1$ vertices). The vertices of the $k$'th block in $N_{i,j}(u)$ will store the $L_{route}(e)$ labels of all the child edges of that block. That is, letting $v_{k,1}, \ldots, v_{k,f+1}$ be the vertices of the $k^{th}$ block, then each $v_{k,\ell}$ stores in its routing table the labels $L_{G,f}(e)$ for $e \in \{ (u,v_{k,1}), \ldots, (u,v_{k,f+1})\}$. The block size is set to be at least $f+1$ in order to make sure that at least one child edge in each block is non-faulty. This is done for every tree $T_{i,j} \in \mathcal{T}$. 
%
%The routing algorithm is also slightly modified. Upon arriving to a vertex $v$ incident to a faulty \emph{tree} edge $e=(u,v)$ the procedure is as follows. Let $T_{i,j}$ be the tree on which $e$ belongs. 
%The index of this tree is specified as part of the succinct path $\widehat{P}$ indicated on the header of the message. Then, if $v$ explicitly stores $L_{route}(e)$ the algorithm works as before. That is, $v$ adds this label to the header, and routes the message back to $s$. Otherwise, $v$ has at least $f+1$ children ($u$ is one of them), and it can locally compute the block of (at least) $f+1$ children to which $u$ belongs. It will then route the message to one of the children of that block (at least one of them is connected to $v$ by a non-faulty edge). That child can then add the labeling information of $e$ to the header of the message, and the message will be routed back to $s$. This completes the description of the modified routing scheme.
We now bound the size of each routing table. 
\begin{claim}
The routing table of each vertex has $\widetilde{O}(f^2 n^{2/k} \log (nW))$ bits.
\end{claim}
\begin{proof}
Each vertex appears in $O(k n^{1/k} \log (nW))$ trees in $\mathcal{T}$. For each such tree, it might store the routing labels of at $O(f)$ edges. Since each label $L_{route}(e)$ has $\widetilde{O}(f n^{1/k} \log (nW))$ bits, over all it stores $\widetilde{O}(f^2 \cdot n^{2/k}\log (nW))$ bits. 
\end{proof}
%The routing procedure is slightly adapted as follows. A vertex $u$ uses the FT-approximate distance labels of its incident edge $e$ only in the case where the routing algorithm asked to send message on $e$ but $e \in F$. In such a case, $u$ routes the message to one of its neighbors in $w$'s block which holds the label of the faulty edge $e$. Note that since $u$ might not know the other faulty edges incident to it, it might approach each of its neighbors in the block of $w$. Since the block has size of $f+1$, at least one of these neighbors should have an non-faulty edge to $u$. 
%
%Since our scheme is based on $(f,8fk)$ FT-approximate distance labels, the stretch is increased by a factor of $2$ compared to the stretch bound of Claim \ref{cl:route-length}. 

\mtodo{how is the stretch affected from the process?}

We have:
\begin{theorem}\label{thm:routing-unknown}[Fault-Tolerant Routing]
For every integers $k,f$, there exists an $f$-sensitive compact routing scheme that given a message $M$ at the source vertex $s$ and a destination $t$, in the presence of at most $f$ faulty edges $F$ (unknown to $s$) routes $M$ from $s$ to $t$ in a distributed manner over a path of length at most $32k f^2\cdot \dist_{G \setminus F}(s,t)$. The table size of each vertex is $\widetilde{O}(f^2 \cdot n^{1/k} \log(nW))$. The header size of the messages is bounded by $\widetilde{O}(f^2)$ bits. 
\end{theorem}

\paragraph{Lower Bound.} Finally, we show that the price of not knowing the set of faulty edges $F$ in advance might indeed incur a multiplicative stretch of $\Omega(f)$. 

\begin{theorem}[Stretch Lower-Bound for FT-Routing]\label{thm:lb-routing}
Any FT-routing randomized scheme resilient to $f$ faults induces an expected stretch of $\Omega(f)$ regardless of the size of the routing tables and labels. In particular, this holds even if each routing table contains a complete information on the graph. 
\end{theorem}
\begin{proof}
Consider a graph that consists of $f+1$ vertex disjoint $s$-$t$ paths, each of length $L=\Theta(n/f)$. The last edge of each of the paths, except for one, is faulty. Assume that the non-faulty path is chosen uniformly at random. Since the routing scheme is oblivious to the faulty edges, it can discover a faulty edge only upon sending the message to one of the edge endpoints. The expected length of the routing is given by:
$$\frac{L}{f+1} +2L \cdot \left(1-\frac{1}{f+1} \right)\cdot \frac{1}{f} + \ldots+ \left(f+1\right)L\cdot \prod_{i=0}^{f-1} \left(1-\frac{1}{f+1-i}\right)=\Omega(f L)~.$$ 
Since the $s$-$t$ shortest path under these faults is $L$, the proof follows. See Fig. \ref{fig:LB-stretch} for an illustration.
\end{proof}


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.40]{lb.pdf}
\caption{\sf Illustration for a stretch lower bound for any FT-routing schemes. The $s$-$t$ pair are connected by $f+1$ vertex disjoint paths. Since the faulty-edge is the last edge of the path, the routing requires $\Omega(L)$ steps to discover a single faulty edge. As the non-faulty path is chosen uniformly at random, in expectation, the routing requires $\Omega(fL)$ steps.  \label{fig:LB-stretch}
}
\end{center}
\end{figure}

%\begin{description}
%\item add the entire label of an edge to the ID of the edge
%\item for the routing scheme have f copies, one per number of current knowledge of faulty edges
%\item in the label of $s$ for every scale $i$ keep the index of the tree that contains the entire $2^i$ ball of $s$. 
%\end{description}
